DecisionPivot: A Diagnostic Benchmark for Decision Models in LLM Systems

Decision models support routing, guardrails, and output verification in LLM systems. However, item accuracy alone cannot establish whether models make correct decisions across controlled variations or assign reliable confidence to their predictions. We introduce DecisionPivot, a diagnostic benchmark comprising 48 tasks and 40,033 items across seven decision roles. Its core track contains 7,800 items from 13 generated task families, organized into contrast groups with computed answers verified by independently implemented solvers. The complementary reference track contains 32,233 items from 35 public test sets, preserving their original evaluation metrics. We evaluate 40 decision models and 14 general models using documented, model-specific protocols, assessing item and contrast-group accuracy, probability ordering, calibration, and empirical selective coverage. Our results reveal substantial differences obscured by aggregate scores: two 27B models separated by only 2.6 points on the reference track achieve contrast-group accuracies of 70.1% and 44.2%. Across 2,400 binary contrast pairs, Perplexity Decider correctly ranks the positive member above the negative member in 92.3% of pairs but answers both members correctly in only 74.1%, exposing a gap between probability ordering and decision correctness. Models with similar item accuracy also differ in the reliability of their high-confidence predictions. On a separate 1,296-item subset, GLM-5.3 achieves 93.5\% contrast-group accuracy at a higher reasoning setting, compared with 81.5% at its lowest effort. By linking errors to pivotal details and difficulty levels, DecisionPivot provides fine-grained diagnostics of decision failures that aggregate evaluation alone cannot reveal.

==> sections/bench_paper_draft.tex <==
\begin{abstract}
Decision models return a probability for each option of a typed question in one forward pass, and
LLM systems act on them at routing, guard and checking points. Converted public test sets no longer
separate the strongest of these models, cannot A what a model has seen, and score only the top
answer. Version 1.1 of DecisionPivot adds 13 program-generated families (7,800 items) of contrast
groups that differ in one planted detail, at three levels, to 35 converted public test sets (34,104
items), under one typed-decision request format. It scores pair accuracy, the share of items a
system can decide alone at an error rate of 5\%, and accuracy at high confidence. Two 27B systems   
0.4 points apart on the public sets reach 46.3 and 70.1 pair accuracy. On six kinds of planted
arithmetic, no one-pass system gets more than 14.3\% of the pairs right. One-pass systems often rank
the two members of a pair correctly yet answer one wrongly, and no single threshold repairs this. A
thought before the answer lifts our 27B reasoning checkpoint from 43.6 to 94.8 pair accuracy, and
general chat models need reasoning as well.
\end{abstract}

\section{Introduction}\label{sec:1}

Besides generating text, an LLM system makes many small decisions: it routes a question, stops an
unsafe prompt, accepts or rejects an answer, checks a tool call before sending it, or rejects a
batch of records that breaks a rule. A decision model answers such a question directly. It reads the
text (the state) and the typed question and returns a probability for every option in one forward
pass, so that the system can decide alone when the model is sure and hand the case on, to a second
look, to more context or to a person, when it is not. A benchmark for these models must ask whether
the answer is right and whether the probability tells when it is.

Existing evaluations convert public test sets, as \citet{deusser2026evaluating} do for a hosted
decision model, and they fall short in three ways. They no longer separate the strongest systems:
our released 27B and Perplexity Decider v1.1 score 57.5 and 57.1 on the 35 converted sets of
DecisionPivot, a paired difference of $-$0.4 points (interval $-$1.3 to +0.5). They cannot show what a
system has seen: one training manifest names the source or a related data set for 16 of these sets,
one model card for 9, and four other systems publish no itemised list. And they score the top answer
only, although five 27B systems whose accuracy differs by 1.9 points can decide between 34.8\% and
42.3\% of our core items alone at an error rate of 5\%.

DecisionPivot answers each shortfall in turn (Figure~\ref{fig:1}). Its \emph{core track} holds 13
families of items written by programs, all of them in \emph{contrast groups}: one case two to four
times, with one \emph{planted detail} that changes the answer (Box~\ref{box:1}), at three levels of
difficulty. The core items are new and their answers computed from the case, so no system has seen
them, and the \emph{reference track} of 35 converted test sets keeps the public sets with the items
found in our training data removed and a flag per system for the data it names. The criteria of use
ask how many groups a system gets wholly right, how much it can decide alone at a fixed error rate,
and how often a confident answer is wrong.

\begin{figure}[!htbp]
\renewcommand{\thefigure}{1}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig1_overview.pdf}
\caption{Both tracks cover the seven layers where a decision sits, and every item reaches a system as one typed request. Left: the core families of each layer and their items, all in contrast groups at three levels. Right: the converted public test sets of each layer and their items, after the removal of the items found in our training data. Bottom: the fields of a request, the reply, and the seven criteria of use. Counts: \texttt{figures/\allowbreak{}fig1\_\allowbreak{}overview.\allowbreak{}csv}, from \texttt{v1\_\allowbreak{}1/\allowbreak{}scores.\allowbreak{}json}.}\label{fig:1}
\end{figure}

\begin{mdbox}{1}{box:1}
\textbf{Box~\ref{box:1}. A contrast pair of \texttt{filter\_\allowbreak{}match} (level 1),
abridged.} The state holds the request and a record of 32 fields, 12 of them shown. The question
asks whether the record satisfies every constraint (options \texttt{no} and \texttt{yes}). The two
members differ only in \texttt{shipping\_\allowbreak{}fee}, which puts the price plus shipping one
cent under or over the limit. No one-pass system gets both members right, and all three of our
reasoning checkpoints do after a thought.

\emph{Request, shared by both members.} ``The listing must satisfy every point below. Its warranty
is not below 36 months. The price plus the shipping fee is less than 500.84 SEK. The price per unit
(bundle price divided by bundle size) is 415.77 SEK or less. The weight is not above 4 kg (the
record gives weights in grams). It ships to Sullis-West. As of 2026-09-10, the listing has been
online for at most 114 days, counted from the listing date. ...''

\emph{Record, fields shared by both members.} Lumrov Mini-404 by Melzim, price 476.80 SEK (list
price 553.09), 10 units for 4,157.70 SEK, warranty 37 months, 3,998 g, listed on 2026-05-19, ships
to Sullis-West among other regions.

\begin{center}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrlrrrr}
\toprule
\textbf{member} & {\begin{tabular}[b]{@{}r@{}}\textbf{shipping}\\\textbf{fee}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{price}\\\textbf{plus}\\\textbf{shipping}\end{tabular}} & \textbf{answer} & {\begin{tabular}[b]{@{}r@{}}\textbf{Perplexity}\\\textbf{Decider}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{our}\\\textbf{released}\\\textbf{27B}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{Clef}\\\textbf{27B}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{our 27B-R,}\\\textbf{with a}\\\textbf{thought}\end{tabular}} \\
\midrule
A & 24.03 & 500.83 & yes & 0.86 & 0.47 & 0.09 & 1.00 \\
B & 24.05 & 500.85 & no & 0.84 & 0.46 & 0.09 & 0.01 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{center}
\end{mdbox}

We ran 27 system configurations in four groups: five open-weight decision models of other groups,
one hosted decision model, 17 checkpoints and read-out modes of our StartLux-Decision family from
0.8B to 27B, and two general chat models with and without reasoning. Five findings stand out, in the
order of the shortfalls. Public sets tie the strongest systems while the core track separates them:
Perplexity Decider and our released 27B lie 0.4 points apart on the reference track and reach 70.1
and 46.3 pair accuracy. Exposure moves the reference track, since our own 4B data rounds gain 8.6
points on reference tasks whose families their data hold and 0.3 on the others. Equal accuracy hides
unequal reliability, and five 27B systems within 1.9 points of accuracy decide 34.8\% to 42.3\% of
the items alone at 5\% error. One-pass models register the planted detail without acting on it, so
that on six kinds of planted arithmetic none gets more than 14.3\% of the pairs right. A thought
before the answer nearly solves the track: our 27B checkpoint rises from 43.6 to 94.8 pair accuracy,
and the chat models need reasoning as well.

DecisionPivot measures whether a decision model reads a written case, acts on the detail that decides
it, and returns a probability that tells a control point when to trust the answer. It does not
measure performance on real traffic, the quality of generated text, other languages, cost or speed.
Our contributions follow the shortfalls: a core track of program-generated contrast groups at three
levels, a reference track with removal of seen items and exposure flags, criteria of use with paired
bootstrap intervals for 27 configurations, a failure analysis that assigns every error to a planted
kind, input-sensitivity tests, and procedural training data with reasoning checkpoints as a matched
reference. Items, generators, solvers, scorer and answer files are released.

\section{Related work}\label{sec:2}

\textbf{Evaluations of decision models.} \citet{deusser2026evaluating} evaluate a hosted decision
model on 37 public data sets with frozen templates, bootstrap intervals, calibration and
selective-prediction measures, and probes that rotate the options. The Decision Index (edition
0.2.1, github.com/apolinario/decision-index) scores 38 public benchmarks into one chance-corrected
index, and JevBench (github.com/fstandhartinger/jevbench) scores calibration, speed and cost on
items authored for it and keeps a sealed sample per release. Both repositories were read on 7
October 2026. None of them computes its answers from a case or scores contrast groups as a whole,
and only JevBench tracks exposure, through its sealed sample and a record of the items sent to
hosted services (Table~\ref{tab:1}).

\textbf{Unified and generated benchmarks.} VBench \citep{huang2023vbench} splits video quality into
16 dimensions with their own evaluation methods, and EmbodiedBench \citep{yang2025embodiedbench}
brings four environments under one framework, as our reference track brings test sets of reward
models \citep{lambert2024rewardbench}, judges \citep{tan2024judgebench}, abstention
\citep{kirichenko2025abstentionbench}, legal classification \citep{guha2023legalbench} and retrieval
\citep{thakur2021beir} under one request format. MineDojo \citep{fan2022minedojo} and StarDojo
\citep{tan2025stardojo} build task suites inside games, as our core track builds cases by program,
and RoboBrain \citep{ji2025robobrain} releases training data and a model next to its evaluation, as
we do with procedural training families and reasoning checkpoints. The bAbI tasks
\citep{weston2015towards} were generated so that every answer is known, GSM-Symbolic
\citep{mirzadeh2024gsm} shows that models answer instances of one template differently, and
LiveBench \citep{white2024livebench} refreshes its questions against contamination.

\textbf{Contrast items, confidence and sensitivity.} Contrast sets \citep{gardner2020evaluating}
perturb an instance so that its label changes, and counterfactually augmented data
\citep{kaushik2019learning} uses the idea for training. Partial-input baselines
\citep{gururangan2018annotation} and heuristic diagnostics \citep{mccoy2019right} show how models
answer from cues. Calibration error \citep{guo2017calibration} and risk-coverage curves
\citep{geifman2017selective} measure whether a confidence can be trusted. The order of the options
\citep{zheng2023large}, irrelevant context \citep{shi2023large} and invariance tests
\citep{ribeiro2020beyond} motivate our input variants.

\begin{table}[!htbp]
\renewcommand{\thetable}{1}
\centering
\caption{\textbf{DecisionPivot and its nearest predecessors}, as described in their papers or documentation. A dash: no such feature found. Computed answers: gold answers computed by a program from the case. Contrast groups: items scored as a group. Exposure control: a means to tell what a system may have seen.}\label{tab:1}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1685}}>{\raggedright\arraybackslash}p{\mdw{0.1269}}>{\raggedright\arraybackslash}p{\mdw{0.1099}}>{\raggedright\arraybackslash}p{\mdw{0.0872}}>{\raggedright\arraybackslash}p{\mdw{0.2027}}>{\raggedright\arraybackslash}p{\mdw{0.1463}}>{\raggedright\arraybackslash}p{\mdw{0.1458}}}
\toprule
\textbf{benchmark} & \textbf{computed answers} & \textbf{contrast groups} & \textbf{levels} & \textbf{criteria beyond accuracy} & \textbf{exposure control} & \textbf{input variants} \\
\midrule
\citet{deusser2026evaluating} & -- & -- & -- & calibration, selective prediction & probes & options rotated \\
Decision Index 0.2.1 & -- & -- & -- & -- & -- & -- \\
JevBench & -- & -- & four tiers & calibration, speed, cost & sealed sample, use record & -- \\
Contrast sets \citep{gardner2020evaluating} & -- & yes & -- & consistency over a set & -- & -- \\
GSM-Symbolic \citep{mirzadeh2024gsm} & yes & -- & added clauses & spread over instances & -- & names, numbers, an irrelevant clause \\
LiveBench \citep{white2024livebench} & partly & -- & -- & -- & new questions each month & -- \\
DecisionPivot (ours) & core track & core track & three & pair accuracy, automation at 5\%, accuracy at 0.90, calibration & own data removed, flags per system & five variants and a rerun \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\section{Tasks}\label{sec:3}

Version 1.1 of DecisionPivot has 48 tasks with 41,904 items in seven layers by where the decision sits
in an LLM system: before generation (A), guards (B), after generation (C), the agent loop (D),
classification that needs reasoning (E), data pipelines (F), and search and matching (G). An item is
a state \emph{s} (a text, or a structure of texts), a question \emph{q} with its type and
instruction, a set of options \emph{O}, each a key with a text, and the gold option \emph{y} in
\emph{O}. A core item adds its contrast group \emph{g}, its level \emph{l} and its planted kind
\emph{k}, the detail the generator changed (none for the unplanted member). A decision model maps
(\emph{s}, \emph{q}, \emph{O}) to a probability for every option in one forward pass, and a
\emph{system} is a model and the way it is run, in one pass or with a thought written before the
read-out. The two tracks trade one strength for another. The core track has exact answers and a
known planted detail in every item, but its cases are invented and their realism is not measured.
The reference track has real text, but its labels carry errors and a system may have trained on its
sources.

\subsection{The core track: 13 generated families}\label{sec:3.1}

\textbf{How an item is made.} A family is a Python script with a fixed seed. It draws a structured
specification of a case (rooms and bookings, a package index and its pins, two ledgers and their
conventions), computes the answer from it and renders the state from the same specification. Names
are invented, sentence types have several phrasings, and every convention the answer depends on is
written in the state, for example whether a limit counts. Each family has 600 items. Six families
were written for version 0 of the benchmark and seven newer ones under stricter rules
(Table~\ref{tab:2}).

\textbf{Contrast groups.} The members of a group share one specification and differ in the planted
detail: in Box~\ref{box:1} the shipping fee, in \texttt{sched\_\allowbreak{}conflict} the opening
time, 07:30 or 07:45, of a room booked from 07:30. Yes/no families have 300 pairs and the families
with three to ten options 150 to 201 groups. The newer families follow written rules. Classes are
balanced exactly, overall and in every level, and so is the position of the gold option. Negatives
are near misses one step beyond a limit, positives sit on the limit or one step inside it as often,
and decoys that look like violations but are not appear in both classes. The members of a group have
the same number of lines and lengths that differ by a few characters in either direction. The
generator asserts that a negative breaks exactly the planted condition, that a positive breaks
nothing, and that no item has a second reading.

\textbf{Levels by what they require.} Level 1 holds few elements of each kind, for example 2 rooms
and 6 to 8 bookings in \texttt{sched\_\allowbreak{}conflict}. Level 2 adds elements and rules to
check. Level 3 needs at least four computation steps or three facts from different places of the
state. In the six older families the level is a size dial of the generator: 4, 8 or 12 policy rules,
30, 60 or 90 log lines, 5, 15 or 25 trace steps, 6, 9 or 12 constraints or schema properties, and in
\texttt{answerable\_\allowbreak{}facts} 2, 3 or 4 facts to combine in a table of 20, 40 or 80 rows.
Each level holds 200 items in every family. The levels were fixed in the generators before any
system ran, except in the four older families rewritten after answers had been seen and in
\texttt{answerable\_\allowbreak{}facts}, whose ladder replaced two crossed dials in version 1.1
(Section~\ref{sec:11}).

\textbf{Checks.} For each family a second author, who had not read the generator, wrote a solver
that sees only the state, the question and the options. It agrees with the generator on all 600
items of every family. The six older families also check every answer against a second engine that
parses the rendered state. In all 13 families, regressions that see only the options or the question
do not beat the majority rate by more than 3 points, and no threshold on the length of a yes/no
state gets beyond 0.50 $\pm$ 0.02 (Appendix~\ref{sec:E}). Two AI reviewers, working apart, answered
65 items of version 1.0 (five per family) from the state before seeing the keys. Both agreed with
all 65 keys. They flagged two \texttt{filter\_\allowbreak{}match} items where a second reading could
flip the key, a paraphrase of the maker constraint and an unstated day-count convention, judged 6 to
10 items natural, 53 to 55 partly natural and 2 to 4 not natural, and listed defects such as
implausible field values. No human audit has been done. Appendix~\ref{sec:A} has a card for every
family.

\textbf{Version 1.1.} This paper describes version 1.1 of 8 October 2026. It keeps the 35 reference
tasks with the same 34,104 items and the scorer and rules of version 1.0, and it again holds 7,800
core items, 600 in each of the 13 families. Ten core families take their items from corrected
generators, which remove the defects the two reviewers listed (Appendix~\ref{sec:E}). Every family
now has a level ladder, and the pairs of \texttt{state\_goal} and
\texttt{toolcall\_\allowbreak{}valid} are marked as contrast groups, so pair accuracy covers all 13
families. The items of \texttt{clause\_\allowbreak{}change}, \texttt{dep\_resolve} and
\texttt{perm\_\allowbreak{}inherit} did not change. An answer file made on the items of version 1.0
does not count for a changed family, so the systems were run again on the ten changed families
(Section~\ref{sec:6.1}).

\begin{table}[!htbp]
\renewcommand{\thetable}{2}
\centering
\caption{\textbf{The 13 core families: no rule that ignores the content comes more than 0.7 points above chance.} Groups: contrast groups (in \texttt{policy\_case} one policy with one case per outcome). Levels: the dial that sets the level, or level where several dials change at once. Rule: best accuracy of a rule that does not read the content, chance in brackets. New in 1.1: the family has new items in version 1.1. State: median characters. Every family has an independent solver that agrees with all 600 keys.}\label{tab:2}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1389}}>{\raggedright\arraybackslash}p{\mdw{0.0656}}>{\raggedright\arraybackslash}p{\mdw{0.2502}}>{\raggedleft\arraybackslash}p{\mdw{0.0869}}>{\raggedleft\arraybackslash}p{\mdw{0.0812}}>{\raggedright\arraybackslash}p{\mdw{0.1153}}>{\raggedleft\arraybackslash}p{\mdw{0.1105}}>{\raggedright\arraybackslash}p{\mdw{0.0744}}>{\raggedleft\arraybackslash}p{\mdw{0.0650}}}
\toprule
\textbf{family} & \textbf{layer} & \textbf{decision} & \textbf{options} & \textbf{groups} & \textbf{levels} & \textbf{rule (chance)} & \textbf{new in 1.1} & \textbf{state} \\
\midrule
\texttt{answerable\_\allowbreak{}facts} & A & can the question be answered from the facts listed & 2 & 300 & facts and rows & 0.507 (0.500) & yes & 2,470 \\
\texttt{perm\_\allowbreak{}inherit} & B & may this user perform this action on this folder & 2 & 300 & level & 0.503 (0.500) & no & 3,926 \\
\texttt{policy\_case} & B & approve, deny or escalate under the written policy & 3 & 201 & rules & 0.333 (0.333) & yes & 1,703 \\
\texttt{log\_\allowbreak{}count\_\allowbreak{}check} & C & is the claimed number of log events right & 2 & 300 & log lines & 0.505 (0.500) & yes & 2,291 \\
\texttt{sched\_\allowbreak{}conflict} & D & can the room booking be confirmed as it stands & 2 & 300 & level & 0.502 (0.500) & yes & 3,029 \\
\texttt{state\_goal} & D & do all goal conditions hold after the agent's trace & 2 & 300 & trace steps & 0.505 (0.500) & yes & 2,475 \\
\texttt{toolcall\_\allowbreak{}valid} & D & is the tool call valid for the schema and the request & 2 & 300 & properties & 0.507 (0.500) & yes & 4,975 \\
\texttt{triage\_\allowbreak{}order} & D & which case do the queue rules put at the asked position & 5 & 201 & level & 0.200 (0.200) & yes & 2,256 \\
\texttt{clause\_\allowbreak{}change} & E & does the change between two versions of an agreement alter the answer & 3 & 201 & level & 0.333 (0.333) & no & 3,730 \\
\texttt{dep\_resolve} & E & does the set of pinned package versions install cleanly & 2 & 300 & level & 0.503 (0.500) & no & 3,348 \\
\texttt{ledger\_\allowbreak{}reconcile} & F & which entry fails to reconcile between two ledgers, or none & 6 & 201 & level & 0.167 (0.167) & yes & 2,764 \\
\texttt{record\_rule} & F & which integrity rule does the batch break, or none & 7 to 10 & 150 & level & 0.122 (0.120) & yes & 4,751 \\
\texttt{filter\_\allowbreak{}match} & G & does the catalogue record meet every constraint & 2 & 300 & constraints & 0.505 (0.500) & yes & 1,647 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\subsection{The reference track: 35 converted test sets}\label{sec:3.2}

Each task is rebuilt by a script from the official files of a public test set and sampled with a
fixed seed, at most 1,000 items (100 queries with 50 candidates for reranking). Thirty-three tasks
keep the labels of their source, and two carry the success rate of a named public chat model,
measured by repeated sampling. We build decision models, so every text field of every converted item
was searched in the 1,546,178 records of our 32 training files, and the 1,234 items found (3.5\% of
35,544) were removed with their groups. Restoring equal classes removed 206 more and left 34,104
items. This protects comparisons among our own checkpoints but says nothing about other systems, so
a flag per task and system records whether the system's published training list names the source
data set or a data set of its family. Appendix~\ref{sec:C} lists every task with its flags.

\section{Interface}\label{sec:4}

A user gets one request per item, sent as it is stored: the \texttt{state} and one question under
the key \texttt{q} with its type, its instruction and its options (\texttt{criteria}, key to text),
in an order frozen in the file. These are the request fields of a typed-decision API, so such a
system runs without any template of ours. A run is one file per task with a probability for every
option key of every item. A failed or missing item counts as wrong, and a run counts only if at
least 99\% of the items have a line and, for a core family, if it was made on the current items,
checked through the hash of the items file. Every item gets one answer from the system's own
probabilities, and nothing is fitted to the benchmark. A chat model is asked for the option key and
a probability for every option, and a system that thinks first reports the read-out after its
thought and keeps the one-pass read-out of the same run as a second system. Appendix~\ref{sec:B}
gives the formats.

\section{Criteria}\label{sec:5}

A control point takes the answer, trusts it when the model is sure, and hands the case on when it is
not. All criteria use the top option of an item (the largest probability, the first listed on a tie)
and its probability. Each criterion catches one failure.

\begin{itemize}
\item \emph{Accuracy}, the share of items whose top option is gold, catches wrong answers but rewards a
system that answers from a cue on one member of each group.
\item \emph{Pair accuracy}, the share of contrast groups with every member right, catches answers from the
surface. In Box~\ref{box:1}, a system that answers yes to both members has accuracy 50.0 and pair
accuracy 0.
\item \emph{Pair direction}, the share of yes/no pairs in which the yes member gets the higher probability
of yes, catches a planted detail that is registered but weighed too little to cross the threshold.
\item \emph{Level-3 pair accuracy}, pair accuracy on the hardest level, catches a reader that loses track
over several steps.
\item \emph{Automation at 5\%} (auto\_at\_5 in the tables), the largest share of the items a system can
decide alone, most confident first, while at most 5\% of them are wrong, catches a probability that
cannot be used to hand cases on.
\item \emph{Accuracy at 0.90} (acc\_at\_090), the accuracy among items whose top probability is at least
0.90, catches confident errors, and the \emph{share at 0.90} says how often the system is that sure.
\item \emph{Calibration error}, the sum over 15 bins of top probability of the gaps between summed
probabilities and right answers, divided by the number of items \citep{guo2017calibration}, catches
probabilities that are too high or too low on average.
\end{itemize}

\textbf{Aggregation, floor and ceiling.} The core headline averages each criterion over the 13
families, which all have contrast groups and a level ladder. On the reference track each task keeps
the metric of its source, turned into a chance-corrected score, 100 $\times$ (value $-$ chance) / (1
$-$ chance), averaged per layer with negative scores counted as 0, and the total is the mean of the
seven layers. Intervals are 95\% percentile bootstrap intervals over contrast groups (1,000
resamples, seed 20261007), with the same draws for every system, so differences between systems are
paired. Table~\ref{tab:3} gives two floors, a uniform guess and the best rule that never reads the
content. The ceiling is a perfect score, since the answers are computed and two independent checks
agree with them.

\section{Results}\label{sec:6}

\subsection{Systems}\label{sec:6.1}

Five open-weight decision models of other groups were run by us from their public weights:
Perplexity Decider v1.1 (27B), Kev 27B, JEV-27B (by its card a student of the hosted reference),
Clef 27B and Clef flash 9.5B. The weights were read at these Hugging Face revisions: Perplexity
Decider v1.1 3b45dea, Kev 27B af0e6d5, JEV-27B 51740a8, Clef 27B 2f3de3d and Clef flash 17f0b0a.
Each model was run by a script of ours that loads it as its card describes (Kev 27B with the
authors' code at commit 5e42a7a, JEV-27B as backbone, adapter and decision head, the Clef models
through their own server), in bf16 on H200 GPUs, one process per GPU. The hosted reference,
jev-1.13.0, was called on 7 October 2026. Its core runs were made on items of version 1.0 in
families that version 1.1 changed, so it appears on the reference track only. Our StartLux-Decision
family \citep{startlux2026report} adds released weights from 0.8B to 27B, checkpoints marked D
(further data rounds aimed at public indices), the untrained starting models of the 4B and 9B, and
checkpoints marked R, trained to write a thought before the read-out. Each R run gives a one-pass
read-out and a read-out after a thought of at most 4,096 tokens on the same items. No D or R
checkpoint is released.

Two general chat models, DeepSeek-V4-Pro and GLM-5.3, answered the core items through their APIs
with the option key and a stated probability for every option (Appendix~\ref{sec:B}), once per item,
and were asked again with the same prompt and parameters on the ten families that version 1.1
changed. Without reasoning they answered all 7,800 items. GLM-5.3 cannot switch reasoning off, and
at its lowest effort it writes a short hidden thought of 121 tokens per item on average. With
reasoning they answered a sample of 1,296 items, 100 per family (99 where groups have three
members), whole groups only and the levels balanced. Their stated top probability is 0.99 or more in
63\% to 97\% of the replies, so they are compared on accuracy, pair accuracy and level 3 only.

\subsection{The reference track ties the leaders}\label{sec:6.2}

Our released 27B (57.5) and Perplexity Decider v1.1 (57.1) lie 0.4 points apart on the reference
track, a paired difference of $-$0.4 points for Perplexity Decider with an interval from $-$1.3 to
+0.5 (layers and tasks in Appendix~\ref{sec:D}). The tie hides layers that go both ways: Perplexity
Decider is ahead by 3.2 points after generation (C) and 3.7 in search and matching (G), and behind
by 3.5 before generation (A) and 4.8 in data pipelines (F), each with a paired interval that
excludes zero. The released 27B is 2.3 points above the hosted reference (paired interval +1.2 to
+3.3) and 4.9 above Clef 27B (+3.9 to +5.9).

\subsection{The core track separates them}\label{sec:6.3}

The core track spreads the same systems over the whole scale (Table~\ref{tab:3} and
Figure~\ref{fig:2}). Among one-pass decision models Perplexity Decider leads with 70.1 pair accuracy
{[}68.7, 71.5{]}, 23.8 points above our released 27B (paired interval 22.2 to 25.5). The other
one-pass 27B systems lie between 43.6 and 47.8, Clef 27B at 24.9, and every smaller one-pass
decision model between 3.8 and 19.2. Scores rise with size, from 3.8 for our released 0.8B and 6.7
at 2B to 13.9 at 4B, 16.2 at 9B and 46.3 at 27B, and decision training adds to them (6.1 for the 4B
starting model). Our data rounds add a little: the 27B-D is 1.5 points above the released 27B
(paired interval 0.1 to 2.8), and the 9B-D and 4B-D are 3.0 and 2.5 points above theirs (1.8 to 4.1
and 1.4 to 3.6). These intervals are over items. A second training run of the 4B round moved pair
accuracy on the version 1.0 items of two families by $-$3.3 and +0.3 points, so the 27B gain lies
within the spread between training runs and the 9B and 4B gains are of about its size. With a
thought, our 27B-R reaches 94.8. Of the chat models, DeepSeek-V4-Pro without reasoning reaches 14.3,
the level of our 4B, because in 8 of the 13 families it gives one answer, no or same, to 72\% to
99\% of the items, and GLM-5.3 with its short thought reaches 82.2. A uniform guess reaches 16.1
pair accuracy and a rule that never reads the content 0.6, and seven systems fall below the guess,
most likely because they give both members of a group the same answer. The gap left is largest on
level 3, where the best one-pass system reaches 57.4 and our 27B-R with a thought 92.4. Per family
(Figure~\ref{fig:3} and Table~\ref{tab:D1}), Perplexity Decider ranges from 97.5 on
\texttt{policy\_case} to 33.8 on \texttt{triage\_\allowbreak{}order}.

\begin{figure}[!htbp]
\renewcommand{\thefigure}{2}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig2_main_results.pdf}
\caption{Three systems within 1.0 point of each other at the top of the reference track lie 23.8 points apart on the core track. Left: pair accuracy on the core track for the systems of Table~\ref{tab:3}, with 95\% bootstrap intervals over contrast groups, and the two floors, a uniform guess (dashed, 16.1) and the best rule that never reads the content (dotted, 0.6). Right: the total of the reference track (0 = chance, 100 = perfect) with 95\% intervals, on the same scale of points per inch, for the systems with runs on all 35 tasks and for the hosted reference, which has no run on the core items of version 1.1. Blue: our checkpoints, orange: other decision models, teal: general chat models. Hatched: a thought before the read-out (for GLM-5.3 the short hidden thought of its lowest effort). Data: \texttt{figures/\allowbreak{}fig2\_\allowbreak{}main\_\allowbreak{}results.\allowbreak{}csv}.}\label{fig:2}
\end{figure}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{3}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig3_family_heatmap.pdf}
\caption{Perplexity Decider leads the other one-pass systems on all 13 families, by less than a point on \texttt{filter\_\allowbreak{}match} and \texttt{ledger\_\allowbreak{}reconcile}, and the 27B-R with a thought stays below 90 only on \texttt{ledger\_\allowbreak{}reconcile} and \texttt{triage\_\allowbreak{}order}. Pair accuracy per core family for the 14 main decision models and the two chat models that answered all 7,800 items, rows sorted by the mean over the 13 families (last column), columns grouped by layer. Data: \texttt{figures/\allowbreak{}fig3\_\allowbreak{}family\_\allowbreak{}heatmap.\allowbreak{}csv}, the values of Table~\ref{tab:D1}.}\label{fig:3}
\end{figure}

\begin{table}[!htbp]
\renewcommand{\thetable}{3}
\centering
\caption{\textbf{Getting it right: one-pass decision models solve 3.8\% to 70.1\% of the contrast groups, our 27B-R with a thought 94.8\%}, over the 13 families, with 95\% bootstrap intervals over contrast groups. Pair accuracy: mean over the 13 families. Level 3: the same on level 3. Values $\times$ 100. D: after data rounds. R: reasoning checkpoint. Chat models: general chat models that state their probabilities, GLM-5.3 with a short hidden thought at its lowest reasoning effort. Last two rows: the floors, a uniform guess (expected values) and the best of three rules that never read the content, chosen per family on its own items (\texttt{v1\_\allowbreak{}1/\allowbreak{}derived/\allowbreak{}floor\_\allowbreak{}rows.\allowbreak{}md}).}\label{tab:3}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrr}
\toprule
\textbf{system} & \textbf{accuracy} & \textbf{pair accuracy} & \textbf{level 3} \\
\midrule
ours 27B-R, with a thought & 97.9 {[}97.6, 98.2{]} & 94.8 {[}94.1, 95.6{]} & 92.4 {[}90.8, 94.0{]} \\
GLM-5.3 (chat model), low reasoning effort & 91.7 {[}91.0, 92.4{]} & 82.2 {[}80.8, 83.7{]} & 75.6 {[}73.0, 78.2{]} \\
Perplexity Decider v1.1 27B & 83.4 {[}82.6, 84.2{]} & 70.1 {[}68.7, 71.5{]} & 57.4 {[}55.2, 59.8{]} \\
ours 9B-R, with a thought & 84.0 {[}83.1, 84.8{]} & 68.0 {[}66.4, 69.6{]} & 47.8 {[}45.5, 50.3{]} \\
ours 4B-R, with a thought & 80.6 {[}79.7, 81.4{]} & 61.0 {[}59.4, 62.6{]} & 42.6 {[}40.2, 45.0{]} \\
ours 27B-D & 72.2 {[}71.2, 73.2{]} & 47.8 {[}46.0, 49.5{]} & 28.4 {[}25.8, 31.1{]} \\
ours 27B, released & 71.7 {[}70.7, 72.7{]} & 46.3 {[}44.6, 48.1{]} & 27.0 {[}24.4, 29.5{]} \\
Kev 27B & 70.6 {[}69.6, 71.6{]} & 44.2 {[}42.6, 46.0{]} & 26.5 {[}24.4, 29.0{]} \\
JEV-27B & 70.3 {[}69.3, 71.4{]} & 44.2 {[}42.6, 45.9{]} & 27.0 {[}24.7, 29.5{]} \\
ours 27B-R, one pass & 70.3 {[}69.4, 71.3{]} & 43.6 {[}41.9, 45.3{]} & 22.6 {[}20.3, 25.0{]} \\
Clef 27B & 60.0 {[}59.1, 61.0{]} & 24.9 {[}23.3, 26.6{]} & 12.8 {[}10.9, 14.7{]} \\
ours 9B-D & 55.7 {[}54.8, 56.6{]} & 19.2 {[}17.8, 20.5{]} & 10.5 {[}8.9, 12.1{]} \\
ours 4B-D & 52.6 {[}51.7, 53.5{]} & 16.4 {[}15.2, 17.6{]} & 7.2 {[}5.8, 8.8{]} \\
ours 9B, released & 54.5 {[}53.7, 55.3{]} & 16.2 {[}15.1, 17.6{]} & 7.7 {[}6.1, 9.3{]} \\
ours 9B-R, one pass & 53.6 {[}52.7, 54.4{]} & 16.1 {[}14.8, 17.3{]} & 9.1 {[}7.3, 10.7{]} \\
DeepSeek-V4-Pro (chat model), no reasoning & 52.7 {[}51.9, 53.6{]} & 14.3 {[}13.2, 15.5{]} & 5.7 {[}4.4, 7.1{]} \\
ours 4B, released & 52.1 {[}51.2, 53.0{]} & 13.9 {[}12.8, 15.1{]} & 5.3 {[}4.1, 6.6{]} \\
Clef flash 9.5B & 50.7 {[}49.8, 51.5{]} & 12.5 {[}11.5, 13.6{]} & 6.2 {[}4.9, 7.6{]} \\
ours 9B starting model & 46.0 {[}45.2, 46.6{]} & 8.4 {[}7.5, 9.4{]} & 3.4 {[}2.5, 4.5{]} \\
ours 2B, released & 44.9 {[}44.2, 45.6{]} & 6.7 {[}5.8, 7.6{]} & 3.3 {[}2.3, 4.4{]} \\
ours 4B starting model & 43.1 {[}42.3, 43.8{]} & 6.1 {[}5.3, 6.8{]} & 4.5 {[}3.4, 5.6{]} \\
ours 0.8B, released & 41.6 {[}41.1, 42.2{]} & 3.8 {[}3.2, 4.4{]} & 2.3 {[}1.6, 3.2{]} \\
uniform guess & 39.6 & 16.1 & 16.1 \\
best rule that never reads the content & 39.9 & 0.6 & 0.2 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\subsection{Same accuracy, different reliability}\label{sec:6.4}

Accuracy does not say how much of the work a system can take over (Table~\ref{tab:4}). Five 27B
systems have accuracy between 70.3 and 72.2, yet at an error rate of at most 5\% they can decide
between 34.8\% (JEV-27B) and 42.3\% (our 27B-D) of the items alone, with intervals that do not
overlap ({[}31.9, 37.6{]} against {[}38.9, 44.2{]}). They also mean different things by sure (top
probability at least 0.90). Kev 27B is sure on 34.1\% of the items and right on 93.8\% of those,
JEV-27B on 47.4\% and right on 88.9\%, so about one in nine of JEV-27B's sure answers is wrong
against one in sixteen for Kev. Calibration error orders them differently again, from 9.2 for Kev
27B to 13.0 for JEV-27B. For a builder, the automation and confidence columns, not accuracy, say how
a model will behave behind a threshold.

\begin{table}[!htbp]
\renewcommand{\thetable}{4}
\centering
\caption{\textbf{Trusting and handing on: five 27B systems within 1.9 points of accuracy decide 34.8\% to 42.3\% of the items alone at 5\% error}, over the 13 families, with 95\% intervals. auto\_at\_5: automation at 5\%, the share of the items a system can decide alone while at most 5\% of them are wrong, mean over families. acc\_at\_090: accuracy at 0.90, the accuracy among the items with top probability at least 0.90, and share\_at\_090 the share of such items, items pooled. Calibration error: 15-bin calibration error, mean over families, shown without an interval. The chat models are left out, as their probabilities are stated, not read out, and the one-pass read-outs of the R checkpoints are in Table~\ref{tab:5}.}\label{tab:4}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrr}
\toprule
\textbf{system} & \textbf{auto\_at\_5} & \textbf{acc\_at\_090} & \textbf{share\_at\_090} & {\begin{tabular}[b]{@{}r@{}}\textbf{calibration}\\\textbf{error}\end{tabular}} \\
\midrule
ours 27B-R, with a thought & 96.9 {[}95.0, 100.0{]} & 98.4 {[}98.1, 98.7{]} & 94.7 {[}94.2, 95.2{]} & 1.9 \\
Perplexity Decider v1.1 27B & 72.3 {[}69.5, 74.1{]} & 92.9 {[}92.1, 93.6{]} & 77.1 {[}76.1, 78.2{]} & 9.3 \\
ours 9B-R, with a thought & 51.3 {[}48.0, 55.7{]} & 92.7 {[}92.1, 93.4{]} & 73.1 {[}72.1, 74.1{]} & 7.2 \\
ours 4B-R, with a thought & 46.2 {[}43.2, 52.5{]} & 90.1 {[}89.3, 90.8{]} & 71.8 {[}70.8, 72.9{]} & 10.1 \\
ours 27B-D & 42.3 {[}38.9, 44.2{]} & 92.5 {[}91.6, 93.3{]} & 45.1 {[}43.9, 46.4{]} & 9.9 \\
ours 27B, released & 41.8 {[}38.4, 44.2{]} & 90.1 {[}89.1, 91.0{]} & 48.6 {[}47.2, 49.9{]} & 11.6 \\
Kev 27B & 35.2 {[}33.2, 38.4{]} & 93.8 {[}93.0, 94.7{]} & 34.1 {[}33.0, 35.5{]} & 9.2 \\
JEV-27B & 34.8 {[}31.9, 37.6{]} & 88.9 {[}87.9, 89.8{]} & 47.4 {[}46.2, 48.8{]} & 13.0 \\
Clef 27B & 14.5 {[}13.4, 17.1{]} & 70.1 {[}68.7, 71.4{]} & 40.8 {[}39.6, 42.1{]} & 22.2 \\
ours 9B-D & 6.6 {[}6.3, 9.5{]} & 77.1 {[}75.3, 78.7{]} & 19.1 {[}18.2, 20.1{]} & 14.6 \\
ours 4B-D & 3.4 {[}3.3, 5.6{]} & 78.0 {[}75.7, 80.2{]} & 12.8 {[}12.0, 13.6{]} & 15.2 \\
ours 9B, released & 6.8 {[}5.6, 8.9{]} & 77.4 {[}75.7, 79.0{]} & 19.3 {[}18.3, 20.3{]} & 16.7 \\
ours 4B, released & 4.0 {[}3.6, 5.8{]} & 71.9 {[}70.0, 73.8{]} & 17.7 {[}16.8, 18.7{]} & 18.4 \\
Clef flash 9.5B & 3.0 {[}2.4, 4.1{]} & 58.2 {[}57.1, 59.2{]} & 33.2 {[}32.2, 34.2{]} & 24.0 \\
ours 9B starting model & 3.3 {[}2.1, 4.5{]} & 61.9 {[}60.4, 63.5{]} & 19.1 {[}18.3, 20.0{]} & 23.6 \\
ours 2B, released & 1.1 {[}0.7, 1.8{]} & 67.1 {[}63.9, 70.6{]} & 4.9 {[}4.4, 5.5{]} & 15.5 \\
ours 4B starting model & 2.0 {[}1.4, 2.9{]} & 67.0 {[}64.5, 69.6{]} & 7.7 {[}7.1, 8.3{]} & 20.2 \\
ours 0.8B, released & 0.2 {[}0.2, 0.5{]} & 61.2 {[}52.8, 69.1{]} & 0.9 {[}0.6, 1.1{]} & 11.6 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\subsection{A thought before the answer}\label{sec:6.5}

Table~\ref{tab:5} compares the one-pass read-out with the read-out after a thought from the same
runs, and with a gate between the two. With 612 thought tokens per item, the 27B reaches 94.8 pair
accuracy and decides 96.9\% of the items alone at the 5\% error rate. The 9B and 4B gain about as
many points, 51.9 and 47.0 against 51.3, but think almost four times as long and stay far below on
level 3 (47.8 and 42.6). A model that reads with care gets nearly every item right, so the low
one-pass scores are not label errors.

A gate that thinks only when the one-pass top probability is below 0.9 keeps most of the gain at
27B. It thinks on 58.0\% of the items, spends 444 thought tokens per item instead of 612, and
reaches 89.3 pair accuracy {[}88.2, 90.3{]}, 5.5 points below a thought on every item (paired
interval $-$6.3 to $-$4.8). The 9B and 4B are sure of so few items in one pass that the gate thinks
on 84.1\% and 88.8\% of them and saves less than a tenth of the tokens. Over thresholds from 0.5 to
0.999 (Figure~\ref{fig:4}), the 27B's pair accuracy climbs steadily with the tokens spent up to
about 0.95 and then flattens.

The chat models need their thought as much (Table~\ref{tab:6}, the sample of 1,296 items). With
reasoning DeepSeek-V4-Pro reaches 99.2 pair accuracy and GLM-5.3 93.5, against 11.6 and 81.5 without
or with little reasoning on the same items. Our 27B-R with a thought (94.4) is 4.7 points below
DeepSeek-V4-Pro (paired interval 2.8 to 6.9) at 606 thought tokens per item against 1,758, and not
distinguishable from GLM-5.3, which spends 265 (GLM-5.3 minus ours $-$0.9, interval $-$3.5 to +1.6).
Its read-out probabilities also let the gate trade accuracy for tokens, to 89.3 at 438 tokens on
these items. On these items the core track is solved by reading with a thought, by decision models
and chat models alike, and by no one-pass reader.

\begin{table}[!htbp]
\renewcommand{\thetable}{5}
\centering
\caption{\textbf{One pass, a gate, and a thought on every item: at 27B the gate keeps 45.7 of the 51.3 points a thought adds, at 73\% of its tokens}, same items and same runs. Gated at 0.9: the read-out after the thought where the one-pass top probability is below 0.9, the one-pass read-out elsewhere. Thinks on: share of items with a thought. Tokens: mean thought tokens per item over all items. Reference: mean chance-corrected score on \texttt{folio\_\allowbreak{}validation}, \texttt{judgebench} and \texttt{processbench}, the reference tasks both read-outs cover. Other columns as in Tables~\ref{tab:3} and \ref{tab:4}.}\label{tab:5}
{\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llrrrrrrrr}
\toprule
\textbf{system} & \textbf{mode} & {\begin{tabular}[b]{@{}r@{}}\textbf{thinks}\\\textbf{on}\end{tabular}} & \textbf{accuracy} & \textbf{pair accuracy} & {\begin{tabular}[b]{@{}r@{}}\textbf{level}\\\textbf{3}\end{tabular}} & \textbf{auto\_at\_5} & {\begin{tabular}[b]{@{}r@{}}\textbf{acc\_at\_090}\\\textbf{(share)}\end{tabular}} & \textbf{tokens} & \textbf{reference} \\
\midrule
ours 27B-R & one pass & 0.0\% & 70.3 & 43.6 {[}41.9, 45.3{]} & 22.6 & 37.0 & 92.5 (42.0) & -- & 63.5 \\
ours 27B-R & gated at 0.9 & 58.0\% & 95.2 & 89.3 {[}88.2, 90.3{]} & 85.1 & 86.2 & 95.4 (95.8) & 444 & 74.8 \\
ours 27B-R & thought & 100.0\% & 97.9 & 94.8 {[}94.1, 95.6{]} & 92.4 & 96.9 & 98.4 (94.7) & 612 & 74.8 \\
ours 9B-R & one pass & 0.0\% & 53.6 & 16.1 {[}14.8, 17.3{]} & 9.1 & 6.6 & 78.6 (15.9) & -- & 50.3 \\
ours 9B-R & gated at 0.9 & 84.1\% & 82.4 & 64.6 {[}62.9, 66.2{]} & 46.2 & 43.8 & 89.8 (75.2) & 2,131 & 59.4 \\
ours 9B-R & thought & 100.0\% & 84.0 & 68.0 {[}66.4, 69.6{]} & 47.8 & 51.3 & 92.7 (73.1) & 2,360 & 59.5 \\
ours 4B-R & one pass & 0.0\% & 51.2 & 14.0 {[}12.8, 15.3{]} & 6.2 & 4.4 & 79.0 (11.2) & -- & 45.0 \\
ours 4B-R & gated at 0.9 & 88.8\% & 79.6 & 59.0 {[}57.3, 60.6{]} & 42.0 & 36.4 & 88.2 (73.0) & 2,116 & 60.8 \\
ours 4B-R & thought & 100.0\% & 80.6 & 61.0 {[}59.4, 62.6{]} & 42.6 & 46.2 & 90.1 (71.8) & 2,271 & 62.0 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{4}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig4_gate_cost.pdf}
\caption{At 27B a gate reaches most of the gain of a thought with fewer tokens, but at 9B and 4B it saves little. Pair accuracy against thought tokens per item (averaged over all items, 0 for an item without a thought) for a gate that thinks when the one-pass top probability is below a threshold. Each curve runs from one pass (left end) to a thought on every item (right end). Small dots: thresholds from 0.5 to 0.999, open markers: 0.9, bars: 95\% intervals. Data: \texttt{figures/\allowbreak{}fig4\_\allowbreak{}gate\_\allowbreak{}cost.\allowbreak{}csv}.}\label{fig:4}
\end{figure}

\clearpage
\begin{table}[!htbp]
\renewcommand{\thetable}{6}
\centering
\caption{\textbf{Reasoning on a sample of 1,296 core items: both chat models need it, DeepSeek-V4-Pro rises from 11.6 to 99.2 pair accuracy} (100 per family, 99 where groups have three members, whole groups, levels balanced). Every system is scored on the same items with shared bootstrap draws. Thought tokens: mean per item (for the gated row over all items, 0 without a thought). Minus 27B-R: paired difference to our 27B-R with a thought, with a 95\% interval. Sources: \texttt{v1\_\allowbreak{}1/\allowbreak{}derived/\allowbreak{}sample\_\allowbreak{}comparison.\allowbreak{}csv} and \texttt{v1\_\allowbreak{}1/\allowbreak{}general\_\allowbreak{}llm/}.}\label{tab:6}
{\scriptsize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrr}
\toprule
\textbf{system} & \textbf{accuracy} & \textbf{pair accuracy} & {\begin{tabular}[b]{@{}r@{}}\textbf{level}\\\textbf{3}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{thought}\\\textbf{tokens}\\\textbf{per item}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{pair accuracy,}\\\textbf{minus 27B-R}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{level 3,}\\\textbf{minus 27B-R}\end{tabular}} \\
\midrule
DeepSeek-V4-Pro (chat model), reasoning on & 99.6 & 99.2 {[}98.2, 99.8{]} & 97.9 & 1,758 & +4.7 {[}+2.8, +6.9{]} & +5.4 {[}+1.2, +9.8{]} \\
GLM-5.3 (chat model), reasoning on & 97.2 & 93.5 {[}91.7, 95.3{]} & 88.3 & 265 & $-$0.9 {[}$-$3.5, +1.6{]} & $-$4.2 {[}$-$9.9, +1.9{]} \\
ours 27B-R, with a thought & 97.5 & 94.4 {[}92.2, 96.3{]} & 92.5 & 606 & -- & -- \\
ours 27B-R, gated at 0.9 & 94.7 & 89.3 {[}86.9, 91.7{]} & 85.1 & 438 & $-$5.1 {[}$-$6.9, $-$3.4{]} & $-$7.4 {[}$-$11.9, $-$3.7{]} \\
ours 9B-R, with a thought & 84.1 & 69.4 {[}65.6, 72.9{]} & 47.0 & 2,356 & $-$25.1 {[}$-$28.8, $-$21.6{]} & $-$45.5 {[}$-$52.9, $-$38.6{]} \\
GLM-5.3 (chat model), low reasoning effort & 91.7 & 81.5 {[}78.4, 84.6{]} & 73.1 & 121 & $-$13.0 {[}$-$16.0, $-$10.0{]} & $-$19.4 {[}$-$25.8, $-$13.0{]} \\
Perplexity Decider v1.1 27B, one pass & 83.6 & 70.4 {[}66.9, 74.0{]} & 56.7 & -- & $-$24.0 {[}$-$27.9, $-$20.3{]} & $-$35.8 {[}$-$42.7, $-$29.1{]} \\
ours 27B, released, one pass & 71.4 & 44.8 {[}40.9, 48.9{]} & 25.1 & -- & $-$49.6 {[}$-$53.5, $-$45.4{]} & $-$67.4 {[}$-$73.1, $-$61.2{]} \\
DeepSeek-V4-Pro (chat model), no reasoning & 51.9 & 11.6 {[}8.9, 14.2{]} & 5.3 & -- & $-$82.9 {[}$-$86.2, $-$79.4{]} & $-$87.2 {[}$-$91.8, $-$82.3{]} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\section{Where today's models fail}\label{sec:7}

Every core item records its level and, in 12 of the 13 families, the kind of its planted detail or
none, so the analysis assigns every error of every decision model to a kind and a level. It counts
all errors on all 7,800 items, not a sample, with paired bootstrap intervals over contrast groups
(\texttt{policy\_case} records no kind and enters by level only).

\textbf{Ranking right, threshold wrong.} On the eight yes/no families, the 18 one-pass decision
models give the yes member the higher probability of yes in 59.3\% to 92.3\% of the pairs but answer
both members right in only 5.7\% to 74.1\% (Table~\ref{tab:7}). Perplexity Decider in
Box~\ref{box:1} is such a case, at 0.86 against 0.84. The planted detail moves the probability the
right way, likely because the models register the difference but weigh it too little against the
rest of the state. No threshold repairs this: one cut on P(yes), fitted on the test pairs themselves
and so an upper bound, raises pair accuracy by 0.1 to 7.8 points, against 18.2\% to 56.4\% of the
pairs ranked right but answered wrong. Recalibrating a threshold will not make these models usable
on such cases, and an evaluator who reports accuracy alone will not see the failure.

\begin{table}[!htbp]
\renewcommand{\thetable}{7}
\centering
\caption{\textbf{Contrast pairs and depth: one-pass models rank most pairs right yet answer both members right in at most 74.1\% of them.} The first five columns are shares of the 2,400 pairs of the eight yes/no families. Best single threshold: pair accuracy with one cut on P(yes) chosen on the same pairs, an upper bound. Level 1, level 3: pair accuracy pooled over the 13 families. Selected systems, the ranges in the text cover all 18 one-pass decision models of the source files \texttt{v1\_\allowbreak{}1/\allowbreak{}analysis/\allowbreak{}out/\allowbreak{}t4\_\allowbreak{}threshold\_\allowbreak{}pooled.\allowbreak{}csv} and \texttt{t2\_\allowbreak{}levels\_\allowbreak{}long.\allowbreak{}csv}.}\label{tab:7}
{\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{system} & \textbf{direction} & {\begin{tabular}[b]{@{}r@{}}\textbf{pair}\\\textbf{accuracy}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{ranked}\\\textbf{right, not}\\\textbf{both right}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{yes member}\\\textbf{answered no}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{pair accuracy,}\\\textbf{best single}\\\textbf{threshold}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{level}\\\textbf{1}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{level}\\\textbf{3}\end{tabular}} \\
\midrule
Perplexity Decider v1.1 27B & 92.3 & 74.1 & 18.2 & 7.9 & 74.2 & 87.7 & 57.4 \\
ours 27B-D & 85.2 & 50.7 & 34.4 & 18.6 & 52.0 & 71.2 & 28.4 \\
ours 27B, released & 84.4 & 48.0 & 36.4 & 25.8 & 51.0 & 70.8 & 27.0 \\
Kev 27B & 84.0 & 45.6 & 38.4 & 26.8 & 47.5 & 66.5 & 26.5 \\
JEV-27B & 82.9 & 48.0 & 34.8 & 18.5 & 48.3 & 66.4 & 27.0 \\
ours 27B-R, one pass & 83.3 & 46.6 & 36.8 & 25.0 & 49.3 & 67.7 & 22.6 \\
Clef 27B & 78.6 & 25.0 & 53.6 & 44.8 & 30.6 & 42.3 & 12.8 \\
ours 9B, released & 73.3 & 17.7 & 55.7 & 41.7 & 23.1 & 29.6 & 7.7 \\
ours 4B, released & 70.1 & 13.9 & 56.2 & 39.1 & 16.9 & 26.2 & 5.3 \\
ours 27B-R, with a thought & 99.2 & 96.8 & 2.4 & 1.0 & 96.9 & 97.3 & 92.4 \\
ours 9B-R, with a thought & 90.3 & 72.7 & 17.6 & 9.9 & 73.1 & 88.5 & 47.8 \\
ours 4B-R, with a thought & 89.5 & 64.8 & 24.7 & 18.3 & 67.6 & 79.2 & 42.6 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\textbf{Doubt is settled on no.} In the pairs ranked right but answered wrong, the wrong answer is
more often a no to the valid member than a yes to the faulty one for 17 of the 18 one-pass systems.
Over the 12 families that mark the planted kind (Table~\ref{tab:8}), every system of the table but
Perplexity Decider and our 27B-R with a thought is more accurate on items with a planted problem
than on items without one, from 4.0 points for our 9B-R with a thought to 48.7 for our 4B starting
model, and by 22.6 for our released 27B (56.6 against 79.2). Perplexity Decider is level (80.9 on
both), and the 27B-R with a thought leans the other way by 1.1 points. A guard built on these models
turns away valid cases more often than it lets faulty ones through, so its rate of false refusals
needs a test of its own.

Whole kinds of planted problem are missed. On the six kinds of \texttt{filter\_\allowbreak{}match}
that need arithmetic on prices or dates (a unit price, a discount, a price plus shipping as in
Box~\ref{box:1}, and three date computations), all 18 one-pass decision models get at most 14.3\% of
the pairs right, with a mean pair direction of 49.6, the level of a coin flip (Figure~\ref{fig:5}).
In \texttt{triage\_\allowbreak{}order} no one-pass system gets more than 5.0\% of the groups right
whose members differ only in the current time, and none that differ in the position asked for, where
the 27B-R with a thought reaches 87.5\% and 93.8\%, and 95.2\% to 100\% on the arithmetic kinds. A
one-pass model should not decide cases that hinge on arithmetic or on a clock, and a builder can
route those to a thought or a tool.

\begin{figure}[!htbp]
\renewcommand{\thefigure}{5}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig5_kinds_pair.pdf}
\caption{No one-pass system solves the kinds that hinge on arithmetic or on the clock. Pair accuracy for the 26 kinds of planted problem with the lowest mean over five systems (kinds with at least 20 items), one panel per system, with 95\% intervals. Bold: the six kinds of \texttt{filter\_\allowbreak{}match} that need arithmetic on prices or dates. Orange: other decision models, blue: our checkpoints, diamonds: a thought before the read-out. Data: \texttt{figures/\allowbreak{}fig5\_\allowbreak{}kinds\_\allowbreak{}pair.\allowbreak{}csv}.}\label{fig:5}
\end{figure}

\textbf{Depth.} Pair accuracy falls from level 1 to level 3 for all 14 main systems, by 4.9 to 43.8
points with paired intervals that exclude zero (Figure~\ref{fig:D1}): from 87.7 to 57.4 for
Perplexity Decider, from 70.8 to 27.0 for our released 27B, and from 97.3 to 92.4 even for the 27B-R
with a thought. A score on short cases overstates a model on long ones, so an evaluator should test
at the depth of the target workload.

\textbf{Confident errors.} Every system is more confident on right than on wrong answers, yet 4.5\%
to 70.5\% of the errors are made at a top probability of 0.90 or more (Table~\ref{tab:8}): 7.1\% of
Kev's, 17.0\% of our released 27B's and 33.2\% of Perplexity Decider's. The 27B-R with a thought
makes only 166 errors in 7,800 items, but 70.5\% of them confidently. A high threshold alone does
not make a model safe to automate, and the share of confident errors belongs next to accuracy in any
report.

\begin{table}[!htbp]
\renewcommand{\thetable}{8}
\centering
\caption{\textbf{Where the errors lie: one-pass models other than Perplexity Decider are more accurate on items with a planted problem than on items without one}, for the 14 main decision models. Accuracy on items without and with a planted problem over the 12 families that mark the planted kind (macro means), the gap with a paired 95\% interval, the kinds of planted problem (of 46 with whole groups and at least 20 items) on which pair accuracy is below 50, the errors among the 7,800 items, and the share of them made at a top probability of 0.90 or more, with a 95\% interval. Sources: \texttt{v1\_\allowbreak{}1/\allowbreak{}analysis/\allowbreak{}out/\allowbreak{}t1\_\allowbreak{}kinds\_\allowbreak{}summary.\allowbreak{}csv} and \texttt{t5\_\allowbreak{}confidence\_\allowbreak{}long.\allowbreak{}csv}.}\label{tab:8}
{\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrr}
\toprule
\textbf{system} & {\begin{tabular}[b]{@{}r@{}}\textbf{no}\\\textbf{planted}\\\textbf{problem}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{planted}\\\textbf{problem}\end{tabular}} & \textbf{gap} & {\begin{tabular}[b]{@{}r@{}}\textbf{kinds below}\\\textbf{50 (pair}\\\textbf{accuracy)}\end{tabular}} & \textbf{errors} & {\begin{tabular}[b]{@{}r@{}}\textbf{errors at 0.90}\\\textbf{or more (share}\\\textbf{of errors)}\end{tabular}} \\
\midrule
ours 27B-R, with a thought & 98.7 & 97.6 & $-$1.1 {[}$-$1.7, $-$0.5{]} & 0 of 46 & 166 & 70.5 {[}63.0, 78.1{]} \\
Perplexity Decider v1.1 27B & 80.9 & 80.9 & +0.1 {[}$-$1.8, +2.2{]} & 14 of 46 & 1,294 & 33.2 {[}30.5, 36.3{]} \\
ours 9B-R, with a thought & 79.7 & 83.8 & +4.0 {[}+2.0, +6.1{]} & 5 of 46 & 1,250 & 33.2 {[}30.4, 35.8{]} \\
ours 4B-R, with a thought & 67.4 & 84.8 & +17.4 {[}+15.6, +19.2{]} & 15 of 46 & 1,514 & 36.7 {[}34.4, 39.3{]} \\
ours 27B-D & 62.4 & 74.2 & +11.8 {[}+9.6, +13.9{]} & 26 of 46 & 2,168 & 12.2 {[}10.9, 13.7{]} \\
ours 27B, released & 56.6 & 79.2 & +22.6 {[}+20.1, +24.9{]} & 28 of 46 & 2,206 & 17.0 {[}15.5, 18.6{]} \\
Kev 27B & 56.5 & 77.5 & +20.9 {[}+18.5, +23.4{]} & 31 of 46 & 2,297 & 7.1 {[}6.2, 8.1{]} \\
JEV-27B & 63.0 & 71.9 & +8.8 {[}+6.3, +11.4{]} & 32 of 46 & 2,316 & 17.8 {[}16.3, 19.3{]} \\
Clef 27B & 32.7 & 76.7 & +43.9 {[}+41.7, +46.1{]} & 44 of 46 & 3,119 & 30.6 {[}29.0, 32.1{]} \\
ours 9B, released & 35.2 & 67.1 & +31.9 {[}+29.6, +34.1{]} & 46 of 46 & 3,547 & 9.6 {[}8.7, 10.6{]} \\
ours 4B, released & 34.6 & 63.2 & +28.5 {[}+26.5, +30.6{]} & 46 of 46 & 3,740 & 10.4 {[}9.5, 11.4{]} \\
Clef flash 9.5B & 28.6 & 65.3 & +36.7 {[}+34.8, +38.6{]} & 43 of 46 & 3,846 & 28.1 {[}27.0, 29.5{]} \\
ours 9B starting model & 27.6 & 63.5 & +35.9 {[}+33.5, +38.3{]} & 46 of 46 & 4,214 & 13.5 {[}12.6, 14.4{]} \\
ours 4B starting model & 18.1 & 66.7 & +48.7 {[}+46.6, +50.7{]} & 46 of 46 & 4,437 & 4.5 {[}3.9, 5.0{]} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\textbf{What a thought fixes and breaks.} The thought fixes 2,187, 2,600 and 2,546 items and breaks
38, 230 and 255 for the 27B-R, 9B-R and 4B-R (Appendix~\ref{sec:D}). At 27B the net gain grows with
depth, from 14.0 points at level 1 to 39.2 at level 3, while the 9B-R and 4B-R gain less at level 3
than at level 1 (24.7 against 33.0 and 30.6). Thoughts cut at the 4,096-token limit, 2,946 at 9B and
2,737 at 4B against 172 at 27B, end in lower accuracy (71.8 and 68.9, against 91.4 and 86.9 on the
other items). Cut thoughts hold 66.6\% and 56.2\% of the errors that remain for the 9B-R and the
4B-R, against 10.8\% for the 27B-R, so for small models the next gain lies in thoughts that end.

\section{What the benchmark measures}\label{sec:8}

\textbf{Reading, not the surface.} No rule that ignores the content comes more than 0.7 points above
chance accuracy on any family, and the best such rule solves 0.6\% of the groups. A model that reads
with a thought solves 94.8\% of them, and the two chat models with reasoning 99.2\% and 93.5\% of
the groups of the sample. The answers lie in the state, and no shortcut we tested reaches them. For
an evaluator, pair accuracy shows answers from the surface that accuracy hides.

\textbf{The two tracks.} The two tracks order the 15 systems that have both nearly alike
(Figure~\ref{fig:D2}). The Spearman correlation between core pair accuracy and the reference total
is 0.97, with a 95\% interval of 0.84 to 1.00 when the systems are resampled and 0.87 to 0.99 when
the core families and the reference tasks are resampled. Where the reference track has run out of
resolution, the core track has not: the three systems within 1.0 point at the top of the reference
track lie 23.8 points apart in pair accuracy. The reference track serves breadth and the core track
the comparison of the strongest systems.

\textbf{Training on the kind of task.} The core items are new for every system, but their kind need
not be. The manifest of Perplexity Decider lists 13 procedural typed-decision families (19.1\% of
its training rows), among them record aggregation and arithmetic. It leads the other one-pass
systems on all 13 families, by 50.7 points on \texttt{dep\_resolve}, a kind its list does not name,
but by only 0.7 on \texttt{filter\_\allowbreak{}match} and 0.5 on
\texttt{ledger\_\allowbreak{}reconcile}, and it gains nothing on the arithmetic kinds of
\texttt{filter\_\allowbreak{}match}, so family names do not explain its margin. None of our
checkpoints in the tables was trained on procedural families. For an evaluator, the names in a
training list are a weak guide to exposure on generated items.

\textbf{Exposure on the reference track.} The published lists show no general lift
(Appendix~\ref{sec:C}). For systems with a list, the score on tasks the list names minus the score
on the others, corrected by the same split for four systems without a list, lies between 0.1 and 6.1
points and excludes zero only for Kev 27B and our released 4B. Our own data rounds give a cleaner
test, because we know what each round added (Table~\ref{tab:9}). A 4B round with training sets from
the families of the reference track's sources gains 8.6 points on the 18 tasks whose families it
holds and 0.3 on the 16 others. The full-coverage round behaves the same way, and a round for weak
areas, which holds none of the 18 families, loses 5.7 points on them. No round raised the tasks
whose families it does not contain, although every item was unseen. A gain on a converted test set
can thus measure exposure, so it should be reported with the exposure next to it.

\begin{table}[!htbp]
\renewcommand{\thetable}{9}
\centering
\caption{\textbf{What three 4B data rounds gain on the reference track}, in points of the chance-corrected score against the 4B-D, whose data mix each round extends, paired over items with 95\% intervals. Covered: the 18 tasks whose families the first two rounds add (preference and judging sets, safety and injection sets, FOLIO, PAWS, AmbigQA, two legal sets and a vulnerable-code set). Other: the 16 tasks whose families none of the three rounds holds. Rounds and numbers from our technical report.}\label{tab:9}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1159}}>{\raggedright\arraybackslash}p{\mdw{0.5971}}>{\raggedleft\arraybackslash}p{\mdw{0.1458}}>{\raggedleft\arraybackslash}p{\mdw{0.1274}}}
\toprule
\textbf{round} & \textbf{data added to the mix of the 4B-D} & \textbf{covered (18 tasks)} & \textbf{other (16 tasks)} \\
\midrule
source families & training sets of the families of the reference track's sources: rating, safety, preference and logic (about 143,000 rows) & +8.6 {[}+7.1, +10.1{]} & +0.3 {[}$-$0.7, +1.3{]} \\
full coverage & the source families, our procedural families, weak-area sets and further task collections & +9.0 {[}+7.3, +10.5{]} & $-$1.3 {[}$-$2.5, 0.0{]} \\
weak areas & training sets for six weak areas of the technical report, none of the 18 families & $-$5.7 {[}$-$7.1, $-$4.5{]} & $-$0.8 {[}$-$1.8, +0.3{]} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\section{Sensitivity to the input}\label{sec:9}

Five variants of the core items, each with the same ids, gold answers and groups, change one thing
that should not matter (Table~\ref{tab:10}). The variants were built from and run on the core items
of version 1.0. Seven one-pass systems were run on them, and a rerun of the original items gives the
noise floor. Option order leaves every score in place: pair accuracy changes by $-$0.7 to +0.3
points with intervals that include zero, accuracy by at most 0.5, and the ranking of the seven
systems by one adjacent swap (our released 27B and the 27B-D) in each file. Single answers do move.
The top option changes on 2.3\% of the items for Perplexity Decider, 4.2\% to 4.9\% for the other
27B systems, 5.6\% for our 9B and 7.9\% to 8.0\% for our 4B, in equal measure from right to wrong
and from wrong to right. Items whose input did not change keep their answer in every system, so the
flips come from the order alone. These numbers cover 12 families, since the reordered
\texttt{log\_\allowbreak{}count\_\allowbreak{}check} runs are missing, and per system they are in
Appendix~\ref{sec:B}. Scores are stable under reordering, but a single decision is not, so a builder
who needs repeatable decisions should fix the order of the options. A paraphrased question moves
pair accuracy by $-$0.9 to +0.6 points, beyond zero only for our released 9B ($-$0.9, interval
$-$1.6 to $-$0.1), and changes the top option on 1.9\% to 5.7\% of the items. An irrelevant
paragraph moves it by $-$1.2 to +0.3, beyond zero only for JEV-27B ($-$1.2, interval $-$2.2 to
$-$0.4), and changes 2.9\% to 7.2\%. Perplexity Decider changes least under both. Cutting the option
texts to bare labels lowers pair accuracy for every system, by 0.4 (Perplexity Decider, with an
interval that includes zero) to 2.8 points, and changes 1.7\% to 9.5\% of the top options, so the
models use the wording of the options. Rewriting the states of eight families as e-mails, tickets or
memos moves pair accuracy by $-$2.4 to +1.3 points, beyond zero only for our released 4B, but
changes the top option on 6.4\% to 20.4\% of the items: a score carries over to natural text while
single answers do not. A rerun of the original items reproduces every answer, so each change above
comes from the input.

\begin{table}[!htbp]
\renewcommand{\thetable}{10}
\centering
\caption{\textbf{Input variants of the core items.} Ids, gold answers and groups are the same in every variant. Seven one-pass systems: our released 27B, 9B and 4B, the 27B-D, Perplexity Decider, Kev 27B and JEV-27B. Results: change of pair accuracy (range over systems, all intervals include zero for option order, one per variant excludes it for the paraphrase and the paragraph) and share of items whose top option changes. Option order reverses half of the yes/no pairs in each file and reorders every item with three or more options. Per system: Appendix~\ref{sec:B}.}\label{tab:10}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1591}}>{\raggedright\arraybackslash}p{\mdw{0.4133}}>{\raggedright\arraybackslash}p{\mdw{0.1192}}>{\raggedleft\arraybackslash}p{\mdw{0.1543}}>{\raggedleft\arraybackslash}p{\mdw{0.1407}}}
\toprule
\textbf{variant} & \textbf{what changes} & \textbf{what it tests} & \textbf{pair accuracy change} & \textbf{top option changes} \\
\midrule
option order (two files) & the order of the options & position bias & $-$0.7 to +0.3 & 2.3\% to 8.0\% \\
paraphrased question & the instruction, one paraphrase per family & wording & $-$0.9 to +0.6 & 1.9\% to 5.7\% \\
irrelevant paragraph & three sentences without facts added to the state & distraction & $-$1.2 to +0.3 & 2.9\% to 7.2\% \\
bare option labels & option texts cut to labels such as ``Yes'' (12 families) & option texts & $-$2.8 to $-$0.4 & 1.7\% to 9.5\% \\
natural text & states of 8 families rewritten by an LLM as e-mails, tickets or memos, every fact checked & form & $-$2.4 to +1.3 & 6.4\% to 20.4\% \\
rerun & nothing & noise floor & 0.0 & 0.0\% \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\section{Matched training data and a stronger reference}\label{sec:10}

We wrote 15 procedural training families in code separate from the benchmark's generators, 135,006
rows with labels computed by the code that builds them: they apply a written policy, count and
aggregate records, track a state, check a call against a specification, chain facts or solve
arithmetic word problems, and rows of one parent group differ in one fact or one claim
\citep{kaushik2019learning}. Their audit mirrors the benchmark's, and no row shares two 13-word
sequences with a core item of version 1.1. On the reference track the 4B round trained on these
families alone is level with the 4B-D ($-$0.5 points, interval $-$1.2 to +0.2), and the
full-coverage round, which adds them among other data, is 0.8 points above it (+0.1 to +1.7), all of
it on the covered tasks. On the version 1.0 items of three core families, the round on our families
alone lifts accuracy from 61.5, 63.2 and 57.2 for the 4B-D to 75.8, 66.3 and 67.0 on answerable
facts, filter match and tool-call validity, and the full-coverage round to 77.3, 66.8 and 68.2, with
the largest gains where a family teaches the kind of the task (multi-hop answerability, a call
checked against a schema). The full-coverage round also trains on data sets from the families of 18
reference tasks, so these tasks are flagged as exposed for it. Our reasoning checkpoints, among them
the strongest decision model on the core track so far, are not released. \todo{release decision for
the R checkpoints and the reasoning server}

\section{Limitations}\label{sec:11}

\begin{enumerate}
\item \textbf{Scope.} DecisionPivot measures reading a written case and the use of a probability at a
control point, not real traffic, generated text, other languages, cost or speed, and every system
was run once.
\item \textbf{Exact answers against realism.} The core track buys exact answers with invented cases. Its
realism was not measured. The two AI reviewers judged most items of version 1.0 only partly natural,
citing template traces such as implausible field values. Version 1.1 removes the traces they listed,
but no reviewer has judged its items again, and no human audit was done. Rewritten as e-mails,
tickets or memos, the items of eight families keep pair accuracy within $-$2.4 to +1.3 points, while
6.4\% to 20.4\% of single answers change. The reference track has real text, but its labels carry
errors we have not measured, and two of its tasks keep a length shortcut (0.729 on \texttt{llmbar},
0.602 on \texttt{bipia\_\allowbreak{}injection}).
\item \textbf{Choices after seeing answers.} Four families of version 0 were written again with harder
dials after three systems' answers had been seen. Version 1.1 changed ten families after the answers
of every system to version 1.0 were known. The changes target the defects the two AI reviewers
listed, and some of them make items harder, such as fewer negatives decided by a cheap check in
\texttt{sched\_\allowbreak{}conflict} and no class-first shortcut in
\texttt{triage\_\allowbreak{}order}.
\item \textbf{The older families.} Independent solvers now check every family, and the older families are
scored as contrast groups like the newer ones, but their generators still take no second seed, so no
sealed set has been drawn from them yet.
\item \textbf{Unknown training data.} The removal of seen items covers our own data only, the exposure
flags rest on published lists, two of them partial and three missing, and nothing is known about the
training data of the two chat models, which were called through a proxy whose weights cannot be
checked.
\item \textbf{Our own interest.} We build the StartLux-Decision models and we built DecisionPivot. The
generators and our training families are separate code checked for overlap, but an outside rerun
would test what we cannot. The items of version 1.1 were frozen on 8 October 2026, before any run of
this paper, and no outside group has rerun them yet.
\end{enumerate}

\section{Release and responsible use}\label{sec:12}

The release holds the core items, the reference items where their licences allow (22 tasks, 4 of
them under share-alike licences) and rebuild scripts for the other 13, the generators, solvers,
audits, scorer, exposure records and answer files. \todo{licence, hosting, DOI, datasheet,
versioning, rule for adding a system, and whether answer files of other systems may be
redistributed} The items are for evaluation only and must not enter the training data or the prompts
of a model in training. Layer B of the reference track holds harmful text by design, as data to
classify. \todo{terms of use for layer B} The core items contain no personal data.

\section{Conclusion}\label{sec:13}

DecisionPivot measures decision models where LLM systems use them. Generated contrast groups separate
the systems that converted public test sets tie, and they show one-pass systems registering a
planted detail without acting on it. A thought before the answer repairs most of this, at hundreds
to thousands of tokens per item. Training families written as code transfer to generated items of
the same kind (answerable facts from 61.5 to 75.8 at 4B) and add nothing to converted public sets
outside their families.

\mdBibliography
\clearpage
\appendix
\section{Task cards of the 13 core families}\label{sec:A}

Every family has 600 items, 200 per level, and one instruction for all of its items. Each card ends
with a contrast from the released items of version 1.1, shortened to the lines that differ. The
README of every family prints one full item per level.

\subsection{\texorpdfstring{\texttt{answerable\_\allowbreak{}facts} (layer A)}{answerable facts (layer A)}}\label{sec:A.1}

\textbf{Question.} ``Can the question be answered from the facts listed?'' Options \texttt{yes}
(every fact the question needs is listed) and \texttt{no}. \textbf{State.} Four rules of reading
(the table is the only source, links between organisations exist only where a parent row names them,
every figure needs its own row, and an organisation without a region row shares the region of its
parent), a table of facts (organisation, attribute, value) about 8, 14 or 26 invented organisations
of two to four families, and a question that needs two, three or four rows, among them totals over
listed subsidiaries and a region taken over from the parent. Every needed row has a near-miss row.
\textbf{Levels.} Level 1: two facts needed in 20 rows, level 2: three in 40, level 3: four in 80. In
40 of the 100 pairs of every level the question needs the region taken over from the parent.
\textbf{Groups.} 300 pairs. The negative replaces one needed row by another attribute of the same
organisation (150) or by the same attribute of a look-alike organisation (150), and changes one
neutral row so that the asked organisation and attribute keep their number of rows. \textbf{Checks.}
Second engine on the rendered text and independent solver, 600 of 600, best content-free rule 0.507.
Second version, harder than version 0. \textbf{Contrast.} ``State the home region of Zolvik Foods.''
Zolvik Foods has no home region row, its parent company row names Zolvik Group, and Zolvik Group has
a home region row (yes). In the other member that row gives the location count of Zolvik Group
instead (no).

\subsection{\texorpdfstring{\texttt{perm\_\allowbreak{}inherit} (layer B)}{perm inherit (layer B)}}\label{sec:A.2}

\textbf{Question.} ``Is the request allowed?'' Options \texttt{yes} and \texttt{no}. \textbf{State.}
The rules of an invented access system written out (assignments reach downward only, group
membership, role extension, action inclusions, sealed folders that cut inheritance from above, deny
entries that beat every allow), the known actions, the inclusion list, roles, users, groups, the
folder tree, role assignments at folders, deny entries and one request. \textbf{Levels.} Level 1:
direct assignments, one group layer, tree depth 2. Level 2: nested groups, one role extension, depth
3, one sealed folder. Level 3: two layers of nesting, extension chains of two, depth 4, two sealed
folders, two or three deny entries and 10 to 14 users, so that the allowing path needs five or more
facts. \textbf{Groups.} 300 pairs. The negative changes one line, the request (150 pairs) or one
line of the structure (150), so that exactly one link of the only allowing path breaks: membership
67, action 67, scope 66, role chain 34, deny 33, sealed folder 33. Decoys in both classes: denies on
sibling folders or for other actions, sealed folders off the path, look-alike names.
\textbf{Checks.} Independent solver 600 of 600 on two seeds. Audit: options alone 0.472, length
0.503, line count 0.500. Fourteen hand-made counts of the structure reach 0.561 in combination, the
best single count 0.548. \textbf{Contrast.} User n.vundarn asks to share at folder
\texttt{invoices}. Role kolkis allows archive, archive includes share, and kolkis is given to group
field-west at the top folder. With field-west's member listed as n.vundarn the request is allowed
(yes), with k.vundarn it is not (no).

\subsection{\texorpdfstring{\texttt{policy\_case} (layer B)}{policy case (layer B)}}\label{sec:A.3}

\textbf{Question.} ``What does the policy require for this case?'' Options \texttt{approve},
\texttt{deny}, \texttt{escalate}, in an order drawn per item. \textbf{State.} A numbered policy of
4, 8 or 12 rules (data export, refunds, access to an internal system and similar) with at least one
exception, a precedence statement (the lower or the higher number wins) and a default, followed by
the case record as \texttt{key: value} lines. A rule that denies or escalates reads a sign of risk
and a rule that approves a sign of low risk, no rule is dead or repeats another, and the fields of a
case agree with each other. \textbf{Levels.} From the number of rules: 4, 8, 12. \textbf{Groups.}
201 policies, 198 with one case per outcome and three with two cases. Outcome, the kind of reading
the case needs (plain, an exception, or the precedence statement, 200 each, each shown by ablation)
and the level are balanced exactly. In 200 items a numeric attribute lies within 5\% of the
threshold that decides the outcome. \textbf{Checks.} A rule engine on the specification, a parser of
the rendered text with a second engine, and an independent solver, 600 of 600. The best content-free
rule reaches 0.333 (chance 0.333). \textbf{Contrast.} Four rules (deny without manager approval,
approve for team Greltis on system classes A to C at clearance 3 or more, escalate below clearance 3
without manager approval, approve during on-call duty), the exceptions that Rule 1 does not apply
during on-call duty and Rule 2 not when the last security training is 365 days old or more, the
lower number wins, the default escalates. A Greltis case at clearance 5 without manager approval:
Rules 1 and 2 apply and Rule 1 wins, so deny. The same team at clearance 4 with approval but
training 665 days ago: the exception removes Rule 2 and no rule applies, so escalate. At clearance 3
with approval and recent training: approve.

\subsection{\texorpdfstring{\texttt{log\_\allowbreak{}count\_\allowbreak{}check} (layer C)}{log count check (layer C)}}\label{sec:A.4}

\textbf{Question.} ``Is the claim correct for this log?'' Options \texttt{yes} and \texttt{no}.
\textbf{State.} An event log of one day with 30, 60 or 90 lines (time, service, level, code) from
four to six invented services, and a claim about the exact number of events of one service and level
in a window, with a stated rule for the end times. \textbf{Levels.} From the number of log lines:
30, 60, 90. \textbf{Groups.} 300 pairs: one log with a true claim and the same log with the claim
changed in one field. The count is off by one (75) or two (75), or the window (75) or the service
(75) is replaced, and then the stated count is the true count of the neighbouring window or of the
other service. Within every level, stated counts of negatives and true counts of positives have the
same histogram (0 to 4, 0 to 8 and 0 to 12 events), so a claim of 0 events is as often true as
false. \textbf{Checks.} Second engine on the rendered text and independent solver, 600 of 600, best
content-free rule 0.505. \textbf{Contrast.} ``svc-dovmora reported exactly 0 INFO events from
09:55:00 until 11:10:00. Both end times count.'' (yes). The same claim with exactly 2 events (no).

\subsection{\texorpdfstring{\texttt{sched\_\allowbreak{}conflict} (layer D)}{sched conflict (layer D)}}\label{sec:A.5}

\textbf{Question.} ``Can the requested booking be confirmed as it stands?'' Options \texttt{yes} and
\texttt{no}. \textbf{State.} Rooms with places, equipment and opening hours, numbered booking
conventions, the confirmed bookings (room, day, time, host, guests) and one request. Bookings of a
room may touch but not overlap, a reset gap applies between bookings from level 2, nobody attends
two overlapping meetings, a booking lies inside the opening hours, host and guests fit the places,
and the room has the equipment asked for. \textbf{Levels.} Rooms 2, 3 to 4, 5 to 6. Bookings 6 to 8,
12 to 16, 20 to 28. Days 1, 1, 2 to 3. Reset gap none, one value, or by kind of room. Requests with
an end time or with a duration. Repeating bookings at level 3. \textbf{Groups.} 300 pairs that
differ in one field, with the positive exactly on the limit that the negative crosses by 5, 10 or 15
minutes, one seat, one item or one person: overlap 112, person 77, hours 48, seats 48, equipment 15.
At levels 2 and 3 the planted rule is mostly a clash in the booking list (overlap or person in 70
and 85 of the 100 negatives of the level), and hours, seats and equipment sit exactly at their
limits in the other pairs. \textbf{Checks.} Independent solver 600 of 600. Audit: options alone
0.464, length 0.502, line count 0.500. Because each positive sits on the limit its negative crosses,
the rule ``the room is exactly full, so yes'' reaches 0.665 at level 1, 0.55 at level 2 and 0.525 at
level 3, though it still needs the seat count and the guest list. \textbf{Contrast.} Room Londa
opens at 07:30, and a booking from 07:30 to 08:45 can be confirmed, since a booking may start at
opening time (yes). In the other member the room opens at 07:45 (no).

\subsection{\texorpdfstring{\texttt{state\_goal} (layer D)}{state goal (layer D)}}\label{sec:A.6}

\textbf{Question.} ``After these operations, are all goal conditions satisfied?'' Options
\texttt{yes} and \texttt{no}. \textbf{State.} The initial content of a small file store (6 to 15
files with ordinary names, from one of five domains such as the pages and settings of a company
website), how each kind of step works (set, delete, rename, copy, move), a goal of 3, 5 or 7
conditions on the final store (a file exists, is absent, holds a content, a folder count, two files
the same) and a numbered trace of steps. Every delete, rename, copy and move finds its file, a set
creates or overwrites one, every step changes the store, and the steps form goal-directed parts of
the work. \textbf{Levels.} From the number of steps: 5, 15, 25. \textbf{Groups.} 300 pairs. One step
of a successful trace is changed so that exactly one condition fails: a wrong target (75), a wrong
content (75), two steps swapped where the order matters (75), or one step left out and another
inserted elsewhere so that the trace keeps its length (75). Both members of a pair hold as many
steps that no condition depends on. Four layouts of the file list, four wordings of the goal and
four step notations are drawn per item. \textbf{Checks.} Simulation on the specification, a second
simulation from the text and an independent solver, 600 of 600, best content-free rule 0.505.
\textbf{Contrast.} The goal asks that \texttt{config/\allowbreak{}menu.\allowbreak{}json} hold
\texttt{default}. The trace sets it to \texttt{stable} and later copies
\texttt{backup/\allowbreak{}menu.\allowbreak{}json}, which holds \texttt{default}, over it (yes). In
the other member the set comes last, after the copy (no).

\subsection{\texorpdfstring{\texttt{toolcall\_\allowbreak{}valid} (layer D)}{toolcall valid (layer D)}}\label{sec:A.7}

\textbf{Question.} ``Is the proposed call correct for the request under this schema?'' Options
\texttt{yes} and \texttt{no}. \textbf{State.} How a call is judged, a tool schema in JSON, a user
request and the proposed call. Schemas have 6, 9 or 12 top-level properties with a nested object, an
array of objects with its own required fields and ranges, one computed parameter (a total or a
count) and one to three rules in the tool description. The request fixes values directly or
indirectly (the last day of a month, the nth weekday, a number of days after a date, quantities at a
price each) and names look-alike identifiers that must not be used. No word of the request equals a
parameter name unless it sets that parameter, and a language is named in words while the call
carries its code. \textbf{Levels.} From the number of properties: 6, 9, 12. \textbf{Groups.} 300
pairs. One planted deviation each, 50 items per kind: a missing required field, a value outside an
enum, a range or the allowed array size, a wrong type, a near miss of a requested value (such as one
day off, two digits transposed, or the look-alike identifier), an undefined field, and a broken rule
of the description. \textbf{Checks.} Second engine on the rendered text and independent solver, 600
of 600, best content-free rule 0.507. Second version, harder than version 0. \textbf{Contrast.} The
request names the reference RF-73392 and warns ``not RF-73932''. The call with RF-73392 is valid
(yes), the call with RF-73932 is not (no).

\subsection{\texorpdfstring{\texttt{triage\_\allowbreak{}order} (layer D)}{triage order (layer D)}}\label{sec:A.8}

\textbf{Question.} ``Which waiting case do the rules put at the position asked for in the state?''
Five options, each a ticket of the queue. \textbf{State.} A service point, the current time,
numbered ordering rules applied in the order given (lower class first, a case waiting at least W
minutes moves up one class but never above class 1, a flagged case counts one class more urgent, due
appointments first, earlier arrival first, shorter handling time first, ticket number last), how
adjustments combine, the queue and the position asked for. No time column contradicts another.
\textbf{Levels.} Cases 6, 9 to 10, 12 to 14. Rules 2 to 3, 4, 5 to 6, with the class as the first
rule at level 1. Class adjustments 0, 1, 2. Position asked 1, 1 to 2, 1 to 3. Half of the waits lie
within 3 minutes of W. \textbf{Groups.} 201 (66 groups of three and one pair per level) on one
queue, differing in one element: an arrival time (217 items), the current time (119), a flag (117),
a listed class (99) or the position asked (48). The five options are the answers of the members and
of plausible misreadings (earliest arrival, highest listed class, one place off, the reversed
tie-break). \textbf{Checks.} Independent solver 600 of 600. The audit on options alone reaches 0.213
against 0.200. At level 1 a reader with the wrong tie-break never gets the key. At levels 2 and 3
the reading ``lowest listed class, then earliest arrival'' gives the key in 12.5\% and 7.5\% of the
items. \textbf{Contrast.} The rules are ``smallest class number first, then earlier arrival, then
lower ticket number''. K-593 and K-602 are both in class 1 and arrived at 09:50, so the ticket
number puts K-593 first. With K-602 arriving at 09:43, K-602 is first.

\subsection{\texorpdfstring{\texttt{clause\_\allowbreak{}change} (layer E)}{clause change (layer E)}}\label{sec:A.9}

\textbf{Question.} ``Does the change between the two versions alter the answer to the point at
issue?'' Options \texttt{same}, \texttt{yes\_only\_A}, \texttt{yes\_only\_B}, 200 each.
\textbf{State.} Rules of reading (each version is complete, clauses correspond by subject and not by
number, and which limit wordings count the stated figure: ``at least'' and ``no more than'' do,
``more than'' and ``under'' do not), versions A and B of an agreement, and a case with facts and a
point at issue. \textbf{Levels.} Clauses per version 8, 10 to 11, 12 to 14. From level 2 a third
changed clause that no case touches and a moved clause, at level 3 an inserted clause and points at
issue that need two clauses. \textbf{Groups.} 201 (66 groups of three and one pair per level) on one
pair of versions: a fact between the old and the new limit of the stricter clause (yes only under
A), a fact between the limits of the looser clause (yes only under B), and a fact outside both bands
(same). The change of a clause is a number (202 items), a wording (199) or both (199). Facts on a
limit, where the wording decides, occur in every class. \textbf{Metric.} Pair accuracy, chance
0.038: a reader who ignores the facts reaches 0.667 per item but solves 1 of 201 groups.
\textbf{Checks.} Independent solver 600 of 600 on two seeds, audit passed. \textbf{Contrast.} The
deposit clause changes from ``more than 32 percent'' to ``at least 40 percent'', the liability
clause from ``under 24000'' to ``under 28000''. A deposit of 40 percent binds the order under both
versions (same). A claim of 24000 is paid in full only under B, so the Manufacturer may decline full
payment only under A (yes\_only\_A).

\subsection{\texorpdfstring{\texttt{dep\_resolve} (layer E)}{dep resolve (layer E)}}\label{sec:A.10}

\textbf{Question.} ``Does the proposed set install cleanly in the target environment?'' Options
\texttt{yes} and \texttt{no}. \textbf{State.} Conventions (versions compare number by number, so
3.10.0 is later than 3.9.9, the meaning of each bound, what a clean install needs, entries of
unpinned versions do not matter, a pin that nothing needs is allowed but its own entry must be met),
the target, the entries of an invented package index with bounds \texttt{\textgreater{}=},
\texttt{\textgreater{}}, \texttt{\textless{}=}, \texttt{\textless{}}, \texttt{==} and \texttt{!=},
required runtimes from level 2, conflicts at level 3, and the pins. \textbf{Levels.} Pins 4 to 5, 6
to 8, 9 to 12. Versions per package 1 to 2, 2 to 3, 3 to 4, so the entry of a pinned version must be
found among look-alikes. Chains of three requirements and conflicts at level 3. \textbf{Groups.} 300
pairs that share every line but one pin: a bound just missed (79, on an excluded bound or the
1.9-against-1.10 trap), a missing pin (78), an unmet requirement of a pinned version (78), the
runtime (45) and a conflict (20). Positives sit on included bounds and just below excluded ones.
\textbf{Checks.} Independent solver 600 of 600 on two seeds. Audit: options alone 0.469, length
0.503, line count 0.500, after the fix of the count of unrequired pins. Level 1 is easy, with a
median of three checks per positive. \textbf{Contrast.} sevdex-odom 4.0.0 needs ostrath-motor
\texttt{!=7.6.6}. Pinning ostrath-motor at 7.4.2 installs cleanly (yes), at 7.6.6 it does not (no).

\subsection{\texorpdfstring{\texttt{ledger\_\allowbreak{}reconcile} (layer F)}{ledger reconcile (layer F)}}\label{sec:A.11}

\textbf{Question.} ``Which entry of ledger A does not reconcile with ledger B?'' Options: five entry
labels of A and \texttt{none}. \textbf{State.} Two ledgers of one period (a stock system against a
receiving log, a cash book against a bank statement), each named one way throughout, the matching
conventions and the statement that at most one entry fails. \textbf{Levels.} Entries per ledger 8,
14, 22. Level 1 pairs entries by reference and equal amounts. Level 2 adds a date tolerance of D
days, split lines whose amounts add up, and opposite signs in B. Level 3 adds a fixed fee per line
of a marked channel, deducted from the size of the figure so that the rule holds for plus and minus
amounts, and batch lines that carry the total of several entries. \textbf{Groups.} 201 (66 groups of
three and one pair per level) on one base, differing only in the planted lines of B. Half of the
groups hold \texttt{none} among their answers, so \texttt{none} is the gold of 100 items. Failure
kinds: missing line 142, amount 140, sign 58, date 57, split sum 56, fee 24, batch total 23.
\textbf{Checks.} Independent solver 600 of 600, options alone 0.146 against 0.167.
\textbf{Contrast.} Ledger B shows $-$280 for the movement that A books as $-$820 (digits
transposed), so A06 fails. In the other member that line agrees and B shows +713 for an entry of
+513, so A02 fails.

\subsection{\texorpdfstring{\texttt{record\_rule} (layer F)}{record rule (layer F)}}\label{sec:A.12}

\textbf{Question.} ``Which rule does the batch violate?'' Options: one key per listed rule (R1 to
Rk, k from 6 to 9, the option text is the rule) and \texttt{none}. \textbf{State.} The fields of a
record type, 6 to 9 numbered integrity rules (3 to 5 of them of kinds that need a computation, two
records or two lists), reference lists with a status per entry, and a batch of records as JSON lines
or a table. The state says that at most one rule is broken, in one place, that whatever no rule
covers is not a violation, and, where a list has a status column, that only a rule naming a status
requires it. Outside the planted violation and one or two deliberate oddities, the fields of every
record agree with each other. \textbf{Levels.} Records per batch 10, 16, 24. \textbf{Groups.} 150
batches with four items each: a near-miss violation of three or four different rules and, in 72
batches, the untouched batch (\texttt{none}, 0.12 of the items). Thirteen rule kinds with 40 or 41
violating items each: a unique key, a reference, a range, a conditional requirement, a date order,
allowed values, a unique pair of fields, a reference to an entry with a given status, a range that
depends on another field, exactly one of two fields, a stored total, a running number and a
reference to an earlier record. Every batch holds a valid look-alike of every listed rule.
\textbf{Checks.} Independent solver 600 of 600, options alone 0.111 against 0.122.
\textbf{Contrast.} The untouched batch (none), the same batch with the mode ``manual'' outside the
allowed values (R5), with an upload date one day before the date taken (R6), and with a repeated
pair of probe and cycle (R1).

\subsection{\texorpdfstring{\texttt{filter\_\allowbreak{}match} (layer G)}{filter match (layer G)}}\label{sec:A.13}

\textbf{Question.} ``Does the record satisfy every constraint of the request?'' Options \texttt{yes}
and \texttt{no}. \textbf{State.} A request in words with 6, 9 or 12 constraints and one catalogue
record in JSON. Ten of the twenty kinds of constraint need a small computation on the record: price
per unit, a discount from the list price, price plus shipping, a unit conversion with the factor
stated, days between two dates, a date plus days, the age of a listing on a stated day, at least k
of n certifications, and a delivery limit that applies only to items shipped from outside a region.
A request that counts days says how, no wording of a constraint can be read as another field of the
record, and the records are plausible (the list price above the price, a bundle at 0.70 to 0.95 of
the unit price, prices and physical specs inside the range of their category). \textbf{Levels.} From
the number of constraints: 6, 9, 12. \textbf{Groups.} 300 pairs. The compared quantity of the
planted constraint lies on the limit or one step from it in both members, a step being one cent, one
gram, one day or one certification. The negative sits on the limit under a wording that does not
count it, or one step beyond. The positive sits on the limit under a wording that counts it, or one
step inside. Computed kinds have 21 negatives each, the others 9. \textbf{Checks.} Second engine on
the rendered text and independent solver, 600 of 600, best content-free rule 0.505. Second version,
harder than version 0. \textbf{Contrast.} ``Its price is 300.80 USD or less.'' A price of 300.79
meets it (yes), 300.81 does not (no).

\section{Protocol details}\label{sec:B}

\textbf{Answer files.} One file per system and task,
\texttt{runs/\allowbreak{}\textless{}system\textgreater{}/\allowbreak{}\textless{}task\textgreater{}.jsonl}.
The short form of a line is \texttt{\{\textquotedbl{}id\textquotedbl{}:
\textquotedbl{}policy\_\allowbreak{}case:00007\textquotedbl{}, \textquotedbl{}p\textquotedbl{}:
\{\textquotedbl{}approve\textquotedbl{}: 0.12, \textquotedbl{}deny\textquotedbl{}: 0.80,
\textquotedbl{}escalate\textquotedbl{}: 0.08\}\}}. The answer object of a typed-decision request is
read as well, including the form \texttt{\{\textquotedbl{}type\textquotedbl{}:
\textquotedbl{}noul\textquotedbl{}, \textquotedbl{}noul\textquotedbl{}: 0.93\}} (the probability of
yes) for yes/no questions. Extra fields are ignored, except that a run with a thought may add
\texttt{tokens} and \texttt{closed} (whether the thought ended by itself). The runners write the
SHA-256 of the items file they ran on next to the answers, and
\texttt{runs\_\allowbreak{}index.\allowbreak{}json} records it for answer files collected from
earlier work.

\textbf{Wording for chat models.} The runner's wording for a chat model that names one key has the
system message ``You answer one typed question about the state you are given. Reply with the key of
exactly one option, copied as it is written, and nothing else.'' The user message holds the state (a
structure as indented JSON) under \texttt{STATE}, the instruction under \texttt{QUESTION}, the
options as \texttt{key: meaning} lines under \texttt{OPTIONS (key: meaning)}, and ends with ``Reply
with one key.'' A reply that names exactly one key gives probability 1 to it, and any other reply
counts as unanswered. The general chat models of Section~\ref{sec:6.1} got the same state, question
and options with two changes that ask for probabilities. The system message reads as follows, and
the user message ends with ``Reply with the JSON object, in this form:'' and the object with the
keys of the item.

\begin{lstlisting}
You answer one typed question about the state you are given. Reply with the key of exactly one
option, copied as it is written, and a probability for every option, as one JSON object and nothing
else: {"choice": "<the key of the option you pick>", "probabilities": {"<key>": <probability>, ...}}.
"probabilities" has one number between 0 and 1 for every option key, the numbers add up to 1, and
each number is how likely you think it is that this option is the right one.
\end{lstlisting}

The top option is the one with the largest stated probability. Without reasoning the requests used
temperature 0 and at most 2,048 (DeepSeek-V4-Pro) or 8,192 (GLM-5.3) output tokens, with reasoning
the provider's default sampling, high effort and at most 32,768 tokens. Version 1.1 kept the replies
of version 1.0 on the three unchanged families and asked again on the ten changed ones with the same
code, prompt and parameters. All 18,192 replies behind the answers of version 1.1 parsed, and no
thought used up the 32,768 tokens. They used 22.9 million prompt tokens and 4.2 million output
tokens
(\texttt{v1\_\allowbreak{}1/\allowbreak{}general\_\allowbreak{}llm/\allowbreak{}run\_\allowbreak{}log.\allowbreak{}txt},
and \texttt{v1/\allowbreak{}general\_\allowbreak{}llm/} for the unchanged families).

\textbf{Runs with a thought.} Each line of a reasoning run holds the one-pass read-out (before the
thought) and the read-out after a thought on every item, with the length of the thought and whether
it ended by itself. A run was taken for a task only if the prompt of at least 99\% of its items
holds the state of the item of version 1.1, the gold answers agree, and at least 99\% of the items
have a line. Runs on the items of version 1.0 of the ten changed families fail the first check and
are not used.

\textbf{The gate.} The gated read-out of Table~\ref{tab:5} takes, item by item, the one-pass
read-out of a reasoning run when its top probability is at least the threshold and the read-out
after the thought otherwise, and counts the thought's tokens only on the items it thinks about. Both
read-outs come from the same run, so the gate needs no further run. Averaging the two read-outs on
the routed items, the default answer of our technical report, is lower at every size (pair accuracy
87.5, 58.8 and 54.0 at 0.9, against 89.3, 64.6 and 59.0). Files:
\texttt{v1\_\allowbreak{}1/\allowbreak{}derived/\allowbreak{}gated\_\allowbreak{}reasoning.\allowbreak{}csv}
and \texttt{v1\_\allowbreak{}1/\allowbreak{}derived/\allowbreak{}gated\_\allowbreak{}runs/}.

\textbf{Worked examples of the criteria.} \emph{aurc}: four items in order of confidence, right,
right, wrong, right, give error rates 0, 0, 1/3 and 1/4 for the prefixes in which they enter, so
aurc = 14.6. \emph{trigger\_recall\_20}: of 10 items with 2 errors, one error among the two least
confident items gives 50.0. \emph{Calibration error}: every item at 0.90 and 70\% right gives 20.0.
\emph{acc\_at\_090}: 5 of 10 items reach 0.90 and 4 of those are right, so acc\_at\_090 is 80.0 with
share 50.0.

\textbf{Intervals.} The bootstrap draws groups where a task has them (pairs, triples, batches,
ranking queries) and items otherwise, with the same draws for every system. Means over families
resample each family. The percentile interval of the calibration error leans upward, with the point
value at its lower end (Kev 27B: 9.2, interval 9.1 to 10.6): the error adds up absolute gaps per
bin, and resampling widens those gaps, so the main text shows no intervals for it. Unit tests of
every score on hand-worked cases are in \texttt{test\_\allowbreak{}score.\allowbreak{}py}.

\textbf{Commands.} \texttt{python3 score.\allowbreak{}py --all --jobs 8} writes
\texttt{scores.json}, \texttt{report.md}, the tables and the list of missing runs. \texttt{bash
refresh.\allowbreak{}sh} rebuilds the task folders, scores everything, writes the registry and runs
the tests.

\begin{table}[!htbp]
\renewcommand{\thetable}{B1}
\centering
\caption{\textbf{Option order per system}, two reordered files of the core items of version 1.0 (12 families, \texttt{log\_\allowbreak{}count\_\allowbreak{}check} missing). Changes: variant minus original in points, for pair accuracy with a 95\% interval over contrast groups (300 resamples). Flips: share of items whose top option changes. Right to wrong and wrong to right: shares of the items in the first file. Source: \texttt{v1/\allowbreak{}sens/\allowbreak{}results/\allowbreak{}sens\_\allowbreak{}table.\allowbreak{}md}.}\label{tab:B1}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrr}
\toprule
\textbf{system} & {\begin{tabular}[b]{@{}r@{}}\textbf{pair accuracy}\\\textbf{change, order 1}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{pair accuracy}\\\textbf{change, order 2}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{accuracy}\\\textbf{change}\\\textbf{(1 / 2)}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{flips (1}\\\textbf{/ 2)}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{right to wrong}\\\textbf{/ wrong to}\\\textbf{right (1)}\end{tabular}} \\
\midrule
Perplexity Decider v1.1 27B & 0.0 {[}$-$0.6, +0.5{]} & $-$0.3 {[}$-$1.0, +0.4{]} & $-$0.1 / 0.0 & 2.3 / 2.3 & 0.9 / 0.8 \\
ours 27B-D & +0.3 {[}$-$0.6, +1.2{]} & $-$0.1 {[}$-$1.0, +0.8{]} & 0.0 / $-$0.1 & 4.5 / 4.2 & 1.6 / 1.6 \\
ours 27B, released & $-$0.4 {[}$-$1.2, +0.5{]} & $-$0.4 {[}$-$1.3, +0.4{]} & $-$0.1 / $-$0.2 & 4.5 / 4.2 & 1.6 / 1.5 \\
Kev 27B & $-$0.5 {[}$-$1.5, +0.6{]} & $-$0.4 {[}$-$1.4, +0.5{]} & $-$0.5 / $-$0.4 & 4.9 / 4.6 & 2.0 / 1.5 \\
JEV-27B & $-$0.1 {[}$-$1.1, +0.8{]} & $-$0.4 {[}$-$1.4, +0.4{]} & +0.1 / $-$0.2 & 4.9 / 4.8 & 1.8 / 1.9 \\
ours 9B, released & $-$0.2 {[}$-$1.0, +0.6{]} & $-$0.3 {[}$-$1.2, +0.5{]} & $-$0.4 / $-$0.5 & 5.6 / 5.6 & 2.1 / 1.7 \\
ours 4B, released & +0.2 {[}$-$0.6, +1.1{]} & $-$0.7 {[}$-$1.5, +0.2{]} & +0.3 / $-$0.3 & 7.9 / 8.0 & 2.4 / 2.7 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\section{Reference tasks and exposure}\label{sec:C}

Table~\ref{tab:C1} sums up the layers, Table~\ref{tab:C2} lists the 35 converted tasks, and
Table~\ref{tab:C3} compares the scores on tasks a training list names with the others. Rule: the
best content-free rule, shown for accuracy tasks only. Ours: share of items found in our training
data before their removal, with tasks at 3\% or more flagged exposed. Perplexity and Kev: own = the
list names the data set, family = it names a data set of the same family, -- = not named, ? =
unknown. Release: I = items included, SA = items included under a share-alike licence, R = rebuild
script only.

The procedural families in the manifest of Perplexity Decider v1.1, with their rows, are arithmetic
(9,227), entity belief tracking (9,232), event-state reconstruction (9,229), evidence sufficiency
(9,214), multi-view adjudication (9,231), needle retrieval (9,225), partial-observation calibration
(9,034), policy applicability (8,925), policy under uncertainty (9,218), record aggregation (9,198),
state perturbation (9,168), table lookup (9,232) and taxonomy routing (9,230). Kev 27B describes
generated policy and rule records, date arithmetic, missing evidence, long states with buried facts
and seven generated families, without publishing the generators. JEV-27B describes 498,010 synthetic
scenarios labelled with the output distributions of the hosted reference and 94,801 programmatic
rows.

\begin{table}[!htbp]
\renewcommand{\thetable}{C1}
\centering
\caption{\textbf{The reference track by layer.} Labels: human / programmatic / mixed. Exposed: tasks flagged exposed (own or family) for our checkpoints, for Perplexity Decider v1.1 and for Kev 27B. The two programmatic tasks of layer A carry success-rate labels of public chat models.}\label{tab:C1}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1577}}>{\raggedleft\arraybackslash}p{\mdw{0.0669}}>{\raggedleft\arraybackslash}p{\mdw{0.0712}}>{\raggedright\arraybackslash}p{\mdw{0.4162}}>{\raggedleft\arraybackslash}p{\mdw{0.0820}}>{\raggedleft\arraybackslash}p{\mdw{0.1929}}}
\toprule
\textbf{layer} & \textbf{tasks} & \textbf{items} & \textbf{two of its decisions} & \textbf{labels} & \textbf{exposed: ours / Perplexity / Kev} \\
\midrule
A before generation & 6 & 5,155 & is the question ambiguous / will a named model answer it correctly & 4 / 2 / 0 & 2 / 2 / 4 \\
B guards & 7 & 3,756 & is the prompt unsafe / does the web page carry an injected instruction & 4 / 2 / 1 & 2 / 4 / 1 \\
C after generation & 8 & 6,018 & which response is better / which step of a solution is the first wrong one & 4 / 1 / 3 & 6 / 4 / 1 \\
D agent loop & 3 & 1,725 & which page element to act on next / did the web agent complete its task & 2 / 0 / 1 & 1 / 0 / 0 \\
E reasoning classification & 4 & 2,466 & does the contract hold a clause of this kind / is the conclusion true, false or undetermined & 2 / 1 / 1 & 2 / 3 / 2 \\
F data pipelines & 1 & 996 & is the label that the data set gives this text correct & 1 / 0 / 0 & 0 / 1 / 1 \\
G search and matching & 6 & 13,988 & do the two records describe the same product / which of two documents that differ by a negation is relevant & 4 / 0 / 2 & 0 / 2 / 0 \\
all & 35 & 34,104 &  & 21 / 6 / 8 & 13 / 16 / 9 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\begingroup
\renewcommand{\thetable}{C2}
\scriptsize\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.1}
\begin{longtable}{>{\raggedright\arraybackslash}p{\mdw{0.1518}}>{\raggedright\arraybackslash}p{\mdw{0.2163}}>{\raggedleft\arraybackslash}p{\mdw{0.0550}}>{\raggedright\arraybackslash}p{\mdw{0.1089}}>{\raggedright\arraybackslash}p{\mdw{0.1070}}>{\raggedleft\arraybackslash}p{\mdw{0.0486}}>{\raggedleft\arraybackslash}p{\mdw{0.0841}}>{\raggedright\arraybackslash}p{\mdw{0.0944}}>{\raggedright\arraybackslash}p{\mdw{0.0556}}>{\raggedright\arraybackslash}p{\mdw{0.0651}}}
\caption{\textbf{The 35 reference tasks.}}\label{tab:C2}\\
\toprule
\textbf{task} & \textbf{decision} & \textbf{items} & \textbf{labels} & \textbf{metric (chance)} & \textbf{rule} & \textbf{ours} & \textbf{Perplexity} & \textbf{Kev} & \textbf{release} \\
\midrule
\endfirsthead
\multicolumn{10}{l}{\textit{Table~\thetable{} (continued)}}\\
\toprule
\textbf{task} & \textbf{decision} & \textbf{items} & \textbf{labels} & \textbf{metric (chance)} & \textbf{rule} & \textbf{ours} & \textbf{Perplexity} & \textbf{Kev} & \textbf{release} \\
\midrule
\endhead
\bottomrule
\endfoot
A \texttt{ambigqa} & does the question have several readings & 998 & human & accuracy (0.500) & 0.553 & -- (0.1\%) & -- & -- & SA \\
A \texttt{cap\_\allowbreak{}boundary\_\allowbreak{}card} & will the named chat model answer correctly & 912 & programmatic & skill (0.000) & -- & exposed (7.9\%) & family & family & R \\
A \texttt{cap\_\allowbreak{}boundary\_\allowbreak{}record} & the same, with the model's record on related questions & 775 & programmatic & skill (0.000) & -- & exposed (21.7\%) & family & family & R \\
A \texttt{freshqa\_\allowbreak{}premise} & does the question rest on a false premise & 498 & human & AUROC (0.500) & -- & -- (0.4\%) & -- & -- & R \\
A \texttt{known\_\allowbreak{}unknown} & does the question have a known answer & 984 & human & accuracy (0.500) & 0.582 & -- (0.8\%) & -- & family & I \\
A \texttt{selfaware} & can the question be answered at all & 988 & human & accuracy (0.500) & 0.571 & -- (0.8\%) & -- & family & SA \\
B \texttt{aegis2\_\allowbreak{}prompt} & is the prompt unsafe & 954 & human & accuracy (0.500) & 0.578 & exposed (3.4\%) & family & own & I \\
B \texttt{bipia\_\allowbreak{}injection} & does the e-mail carry an inserted instruction & 88 & programmatic & accuracy (0.500) & 0.602 & -- (0.0\%) & family & -- & I \\
B \texttt{browsesafe} & does the web page carry an injected instruction & 1,000 & programmatic & accuracy (0.500) & 0.506 & -- (0.0\%) & ? & -- & I \\
B \texttt{cosapien\_\allowbreak{}policy} & allowed, disallowed or partly allowed under a safety configuration & 148 & human & accuracy (0.333) & 0.432 & -- (0.0\%) & -- & -- & I \\
B \texttt{jailbreak\_\allowbreak{}wild} & is the prompt a jailbreak attempt & 824 & mixed & accuracy (0.500) & 0.525 & exposed (11.9\%) & family & -- & I \\
B \texttt{jbb\_judge} & does the response give harmful content & 293 & human & AUROC (0.500) & -- & -- (2.3\%) & -- & -- & I \\
B \texttt{xstest} & should the request be refused & 449 & human & AUROC (0.500) & -- & -- (0.2\%) & family & -- & I \\
C \texttt{contextual\_\allowbreak{}judge} & which response is better for the context & 894 & mixed & accuracy (0.500) & 0.503 & exposed (10.6\%) & -- & -- & I \\
C \texttt{faithbench} & is the summary faithful to its source & 304 & human & accuracy (0.500) & 0.549 & exposed (4.0\%) & -- & -- & R \\
C \texttt{judgebench} & which response is correct & 619 & programmatic & accuracy (0.500) & 0.549 & -- (0.0\%) & -- & -- & I \\
C \texttt{llmbar} & which output follows the instruction better & 399 & human & accuracy (0.500) & 0.729 & exposed (4.8\%) & family & -- & I \\
C \texttt{processbench} & which step is the first wrong one, or none & 966 & human & accuracy (0.142) & 0.367 & exposed (3.4\%) & family & family & I \\
C \texttt{rewardbench} & which response is better & 912 & mixed & accuracy (0.500) & 0.553 & exposed (8.8\%) & family & -- & R \\
C \texttt{rewardbench2} & which of four responses is best & 980 & mixed & accuracy (0.250) & 0.350 & -- (2.0\%) & family & -- & I \\
C \texttt{squad2\_\allowbreak{}answerable} & can the question be answered from the passage & 944 & human & accuracy (0.500) & 0.543 & exposed (4.9\%) & ? & -- & SA \\
D \texttt{agentreward\_\allowbreak{}success} & did the web agent complete its task & 552 & human & accuracy (0.500) & 0.549 & -- (0.2\%) & -- & -- & R \\
D \texttt{bfcl\_\allowbreak{}relevance} & does any listed function serve the request & 176 & mixed & accuracy (0.500) & 0.557 & exposed (22.4\%) & -- & -- & I \\
D \texttt{mind2web\_\allowbreak{}element} & which of ten page elements to act on next & 997 & human & accuracy (0.100) & 0.113 & -- (0.3\%) & -- & -- & R \\
E \texttt{cuad\_clause} & does the contract hold a clause of the named category & 320 & human & accuracy (0.500) & 0.584 & exposed (42.3\%) & family & family & I \\
E \texttt{folio\_\allowbreak{}validation} & is the conclusion true, false or undetermined & 204 & human & accuracy (0.333) & 0.353 & -- (0.0\%) & own & -- & SA \\
E \texttt{legalbench\_\allowbreak{}mix} & ten legal classification sub-tasks & 942 & mixed & accuracy (0.428) & 0.451 & exposed (5.8\%) & family & family & I \\
E \texttt{primevul\_\allowbreak{}pair} & is the function vulnerable (asked for a function and its patch) & 1,000 & programmatic & pair accuracy (0.250) & -- & -- (0.0\%) & -- & -- & I \\
F \texttt{label\_\allowbreak{}errors} & is the label of the text correct & 996 & human & accuracy (0.500) & 0.524 & -- (0.0\%) & family & own & R \\
G \texttt{entity\_\allowbreak{}match\_\allowbreak{}abt\_\allowbreak{}buy} & do the two records describe the same product & 996 & mixed & AUROC (0.500) & -- & -- (0.4\%) & -- & -- & R \\
G \texttt{entity\_\allowbreak{}match\_\allowbreak{}amazon\_\allowbreak{}google} & do the two records describe the same product & 1,000 & mixed & AUROC (0.500) & -- & -- (0.0\%) & -- & -- & R \\
G \texttt{nevir} & which of two documents that differ by a negation is relevant & 1,000 & human & pair accuracy (0.250) & -- & -- (0.0\%) & family & -- & I \\
G \texttt{paws} & do the two sentences mean the same & 992 & human & accuracy (0.500) & 0.538 & -- (0.6\%) & -- & -- & R \\
G \texttt{rerank\_\allowbreak{}nfcorpus} & how well does the passage answer the query & 5,000 & human & nDCG@10 (0.140) & -- & -- (0.0\%) & -- & -- & R \\
G \texttt{rerank\_\allowbreak{}scifact} & how well does the passage answer the query & 5,000 & human & nDCG@10 (0.090) & -- & -- (0.0\%) & family & -- & R \\
\end{longtable}
\endgroup

\begin{table}[!htbp]
\renewcommand{\thetable}{C3}
\centering
\caption{\textbf{Exposure flags on the reference track: the corrected gap excludes zero only for Kev 27B and our released 4B.} Named: tasks whose source data set, or a data set of its family, the published training list names (for our checkpoints, our own training data). Mean: chance-corrected score floored at 0, averaged over the tasks. Gap: named minus not named, with a 95\% interval over 1,000 resamples of the tasks. Controls: the four systems without a published list, the hosted reference, Clef 27B, Clef flash 9.5B and JEV-27B. Gap of the controls: the same split for them. Corrected gap: gap minus the gap of the controls. Two tasks of Perplexity Decider are unknown. Source: \texttt{v1/\allowbreak{}analysis/\allowbreak{}out/\allowbreak{}t7\_\allowbreak{}exposure.\allowbreak{}csv}, valid for version 1.1 since the reference items and their runs did not change.}\label{tab:C3}
{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llrrrrrr}
\toprule
\textbf{system} & \textbf{list} & {\begin{tabular}[b]{@{}r@{}}\textbf{tasks}\\\textbf{named /}\\\textbf{not named}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{mean}\\\textbf{named}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{mean}\\\textbf{not}\\\textbf{named}\end{tabular}} & \textbf{gap} & {\begin{tabular}[b]{@{}r@{}}\textbf{gap of}\\\textbf{the}\\\textbf{controls}\end{tabular}} & \textbf{corrected gap} \\
\midrule
Perplexity Decider v1.1 27B & manifest & 16 / 17 & 63.9 & 58.7 & +5.2 {[}$-$16.0, +25.4{]} & +3.3 & +1.8 {[}$-$3.8, +7.7{]} \\
Kev 27B & model card & 9 / 26 & 48.0 & 60.9 & $-$12.9 {[}$-$30.4, +4.1{]} & $-$18.6 & +5.7 {[}+0.8, +11.3{]} \\
ours 27B, released & our data & 13 / 22 & 55.0 & 65.3 & $-$10.3 {[}$-$25.6, +9.0{]} & $-$10.9 & +0.6 {[}$-$4.1, +4.9{]} \\
ours 27B-D & our data & 13 / 22 & 53.0 & 63.8 & $-$10.9 {[}$-$27.1, +9.1{]} & $-$10.9 & +0.1 {[}$-$5.0, +5.3{]} \\
ours 9B, released & our data & 13 / 22 & 50.6 & 58.7 & $-$8.1 {[}$-$24.4, +11.0{]} & $-$10.9 & +2.8 {[}$-$1.4, +7.0{]} \\
ours 4B, released & our data & 13 / 22 & 50.1 & 55.0 & $-$4.8 {[}$-$21.7, +14.3{]} & $-$10.9 & +6.1 {[}+1.3, +11.1{]} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\section{Full results}\label{sec:D}

The full tables of version 1.1, with every score of every system per family and per task, are in
\texttt{external/\allowbreak{}bench/\allowbreak{}v1\_\allowbreak{}1/\allowbreak{}report.\allowbreak{}md}.
Table~\ref{tab:D1} gives the core track per family, Table~\ref{tab:D2} the reference track per
layer, Table~\ref{tab:D3} the chance-corrected score per reference task for the leading systems, and
Table~\ref{tab:D4} what a thought fixes and breaks.

\begin{table}[!htbp]
\renewcommand{\thetable}{D1}
\centering
\caption{\textbf{Core track per family: the 27B-R with a thought stays below 90 pair accuracy only on \texttt{ledger\_\allowbreak{}reconcile} and \texttt{triage\_\allowbreak{}order}.} Pair accuracy in every family. AF \texttt{answerable\_\allowbreak{}facts}, CC \texttt{clause\_\allowbreak{}change}, DR \texttt{dep\_resolve}, FM \texttt{filter\_\allowbreak{}match}, LC \texttt{log\_\allowbreak{}count\_\allowbreak{}check}, LR \texttt{ledger\_\allowbreak{}reconcile}, PC \texttt{policy\_case}, PI \texttt{perm\_\allowbreak{}inherit}, RR \texttt{record\_rule}, SC \texttt{sched\_\allowbreak{}conflict}, SG \texttt{state\_goal}, TO \texttt{triage\_\allowbreak{}order}, TV \texttt{toolcall\_\allowbreak{}valid}. The hosted reference and the two further 4B checkpoints of Table~\ref{tab:D2} have no runs on the items of version 1.1.}\label{tab:D1}
{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
\textbf{system} & \textbf{AF} & \textbf{CC} & \textbf{DR} & \textbf{FM} & \textbf{LC} & \textbf{LR} & \textbf{PC} & \textbf{PI} & \textbf{RR} & \textbf{SC} & \textbf{SG} & \textbf{TO} & \textbf{TV} \\
\midrule
ours 27B-R, with a thought & 95.7 & 96.0 & 97.3 & 99.3 & 99.0 & 82.6 & 97.5 & 92.3 & 94.7 & 96.3 & 96.0 & 87.6 & 98.7 \\
GLM-5.3 (chat model), low reasoning effort & 92.7 & 93.0 & 91.7 & 96.0 & 74.0 & 69.7 & 81.6 & 69.3 & 78.7 & 72.3 & 78.7 & 74.6 & 97.0 \\
Perplexity Decider v1.1 27B & 92.0 & 96.0 & 94.7 & 37.3 & 72.0 & 41.3 & 97.5 & 78.7 & 50.0 & 51.3 & 76.7 & 33.8 & 90.0 \\
ours 9B-R, with a thought & 67.3 & 77.6 & 62.3 & 93.3 & 84.7 & 41.3 & 88.1 & 59.7 & 37.3 & 60.7 & 75.0 & 57.7 & 78.7 \\
ours 4B-R, with a thought & 71.3 & 66.7 & 45.3 & 94.3 & 80.7 & 57.2 & 83.6 & 53.7 & 16.7 & 63.0 & 69.3 & 51.2 & 40.3 \\
ours 27B-D & 69.7 & 63.2 & 44.0 & 36.7 & 34.7 & 39.3 & 48.3 & 44.7 & 38.7 & 38.0 & 57.3 & 25.4 & 81.0 \\
ours 27B, released & 71.7 & 66.7 & 40.3 & 21.0 & 33.0 & 40.8 & 44.3 & 48.0 & 37.3 & 38.0 & 51.3 & 28.9 & 80.3 \\
Kev 27B & 68.3 & 60.7 & 38.7 & 20.7 & 36.7 & 39.3 & 44.3 & 42.3 & 41.3 & 28.7 & 51.0 & 24.4 & 78.7 \\
JEV-27B & 72.0 & 59.2 & 41.7 & 26.0 & 31.7 & 36.3 & 35.8 & 34.0 & 34.7 & 36.0 & 56.3 & 24.4 & 86.7 \\
ours 27B-R, one pass & 66.3 & 53.7 & 40.3 & 30.0 & 28.0 & 36.3 & 45.3 & 44.3 & 33.3 & 33.3 & 57.0 & 25.4 & 73.3 \\
Clef 27B & 39.3 & 26.4 & 12.3 & 14.3 & 10.7 & 31.3 & 27.9 & 29.0 & 22.7 & 21.7 & 27.7 & 15.4 & 45.0 \\
ours 9B-D & 26.3 & 17.9 & 14.7 & 25.0 & 26.0 & 21.9 & 13.4 & 25.0 & 2.0 & 10.7 & 18.7 & 10.0 & 38.3 \\
ours 4B-D & 25.3 & 15.9 & 13.7 & 28.0 & 18.7 & 20.9 & 20.4 & 19.3 & 1.3 & 9.3 & 13.3 & 12.4 & 14.7 \\
ours 9B, released & 33.0 & 20.4 & 9.3 & 15.3 & 10.3 & 18.9 & 15.9 & 23.3 & 4.7 & 11.7 & 20.7 & 10.0 & 17.7 \\
ours 9B-R, one pass & 20.3 & 15.4 & 12.7 & 20.7 & 13.0 & 21.9 & 13.4 & 20.0 & 8.0 & 5.7 & 15.7 & 11.9 & 31.0 \\
DeepSeek-V4-Pro (chat model), no reasoning & 31.7 & 0.0 & 13.3 & 18.7 & 1.0 & 28.9 & 9.5 & 13.3 & 15.3 & 2.7 & 12.3 & 6.5 & 33.3 \\
ours 4B, released & 28.0 & 17.9 & 8.7 & 16.0 & 2.7 & 19.9 & 18.9 & 19.0 & 3.3 & 7.0 & 18.0 & 10.0 & 11.7 \\
Clef flash 9.5B & 23.7 & 9.0 & 6.0 & 3.7 & 0.0 & 13.4 & 19.9 & 21.3 & 0.7 & 5.0 & 11.3 & 8.5 & 40.7 \\
ours 9B starting model & 20.3 & 0.0 & 2.0 & 17.3 & 6.3 & 9.0 & 6.5 & 11.3 & 0.7 & 3.0 & 12.7 & 1.0 & 19.7 \\
ours 2B, released & 13.0 & 0.5 & 7.3 & 8.3 & 3.3 & 6.0 & 6.5 & 12.3 & 0.0 & 3.3 & 9.7 & 3.0 & 14.0 \\
ours 4B starting model & 18.3 & 4.5 & 2.0 & 7.0 & 0.0 & 1.0 & 4.0 & 17.0 & 0.0 & 16.3 & 5.7 & 0.5 & 2.7 \\
ours 0.8B, released & 5.0 & 0.5 & 4.7 & 2.3 & 5.7 & 0.0 & 3.5 & 7.7 & 0.0 & 1.0 & 8.0 & 0.5 & 11.0 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\begin{table}[!htbp]
\renewcommand{\thetable}{D2}
\centering
\caption{\textbf{Reference track: chance-corrected score per layer and total} (0 = chance, 100 = perfect). A layer is the mean of its task scores floored at 0, the total the mean of the seven layers. D: after data rounds. R: reasoning checkpoint, read out here in one pass by the plain runner. RL: the 4B-D trained further with reinforcement learning. The hosted reference's two reranking tasks hold the ranking published by the source test's authors.}\label{tab:D2}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{system} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{E} & \textbf{F} & \textbf{G} & \textbf{total} \\
\midrule
ours 27B, released & 39.2 & 79.3 & 58.3 & 74.9 & 49.2 & 26.7 & 74.6 & 57.5 \\
Perplexity Decider v1.1 27B & 35.7 & 77.1 & 61.5 & 74.0 & 51.1 & 21.9 & 78.3 & 57.1 \\
ours 27B-D & 36.2 & 77.5 & 55.1 & 73.0 & 50.5 & 29.3 & 73.7 & 56.5 \\
hosted reference (jev-1.13.0) & 36.5 & 79.6 & 59.5 & 66.7 & 50.6 & 21.3 & 72.1 & 55.2 \\
JEV-27B & 41.7 & 71.4 & 57.1 & 69.7 & 46.6 & 23.1 & 71.5 & 54.4 \\
Kev 27B & 39.2 & 70.1 & 52.7 & 70.0 & 48.7 & 24.9 & 73.0 & 54.1 \\
ours 9B-D & 35.6 & 69.7 & 50.1 & 69.8 & 44.6 & 32.9 & 68.9 & 53.1 \\
ours 9B, released & 34.7 & 72.1 & 49.9 & 71.1 & 44.2 & 29.9 & 69.5 & 53.1 \\
Clef 27B & 33.1 & 76.3 & 50.4 & 64.9 & 44.6 & 26.7 & 72.0 & 52.6 \\
ours 4B-D, then RL & 31.5 & 68.5 & 47.8 & 67.3 & 43.2 & 29.7 & 68.2 & 50.9 \\
ours 4B-D & 31.5 & 68.1 & 47.6 & 66.2 & 42.9 & 29.5 & 68.3 & 50.6 \\
ours 4B, released & 31.6 & 69.0 & 48.5 & 67.8 & 43.9 & 27.1 & 65.8 & 50.5 \\
ours 4B-R, one pass (plain runner) & 25.4 & 66.9 & 43.9 & 64.7 & 43.4 & 28.1 & 66.4 & 48.4 \\
Clef flash 9.5B & 32.5 & 68.2 & 39.7 & 63.5 & 39.4 & 25.7 & 67.7 & 48.1 \\
ours 9B starting model & 29.5 & 69.3 & 43.5 & 63.2 & 39.9 & 17.1 & 58.9 & 45.9 \\
ours 2B, released & 23.5 & 60.5 & 35.6 & 66.2 & 38.6 & 26.9 & 64.9 & 45.2 \\
ours 4B starting model & 27.3 & 65.2 & 36.3 & 55.6 & 37.5 & 3.2 & 61.4 & 40.9 \\
ours 0.8B, released & 15.9 & 48.1 & 25.5 & 62.5 & 29.9 & 28.3 & 56.3 & 38.1 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\begingroup
\renewcommand{\thetable}{D3}
\scriptsize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}
\begin{longtable}{llrrrrrrr}
\caption{\textbf{Chance-corrected score per reference task} for seven systems (0 = chance, 100 = perfect, negative values kept). Skill: the skill score against success-rate labels. Hosted: the hosted reference.}\label{tab:D3}\\
\toprule
\textbf{task} & \textbf{metric} & {\begin{tabular}[b]{@{}r@{}}\textbf{ours}\\\textbf{27B}\end{tabular}} & \textbf{Perplexity} & {\begin{tabular}[b]{@{}r@{}}\textbf{ours}\\\textbf{27B-D}\end{tabular}} & \textbf{hosted} & \textbf{JEV-27B} & \textbf{Kev} & {\begin{tabular}[b]{@{}r@{}}\textbf{Clef}\\\textbf{27B}\end{tabular}} \\
\midrule
\endfirsthead
\multicolumn{9}{l}{\textit{Table~\thetable{} (continued)}}\\
\toprule
\textbf{task} & \textbf{metric} & {\begin{tabular}[b]{@{}r@{}}\textbf{ours}\\\textbf{27B}\end{tabular}} & \textbf{Perplexity} & {\begin{tabular}[b]{@{}r@{}}\textbf{ours}\\\textbf{27B-D}\end{tabular}} & \textbf{hosted} & \textbf{JEV-27B} & \textbf{Kev} & {\begin{tabular}[b]{@{}r@{}}\textbf{Clef}\\\textbf{27B}\end{tabular}} \\
\midrule
\endhead
\bottomrule
\endfoot
A \texttt{ambigqa} & accuracy & 8.2 & 4.0 & 3.6 & 28.9 & 26.3 & 5.6 & 5.4 \\
A \texttt{cap\_\allowbreak{}boundary\_\allowbreak{}card} & skill & 6.1 & 9.4 & $-$42.0 & 4.9 & 23.3 & 21.3 & $-$2.4 \\
A \texttt{cap\_\allowbreak{}boundary\_\allowbreak{}record} & skill & 29.2 & 17.5 & 28.8 & 23.9 & 29.8 & 27.9 & 6.3 \\
A \texttt{freshqa\_\allowbreak{}premise} & auroc & 86.3 & 91.2 & 85.9 & 88.2 & 85.1 & 84.2 & 84.5 \\
A \texttt{known\_\allowbreak{}unknown} & accuracy & 71.1 & 72.6 & 71.7 & 55.1 & 57.5 & 70.1 & 70.9 \\
A \texttt{selfaware} & accuracy & 34.4 & 19.4 & 27.3 & 18.0 & 27.9 & 26.3 & 31.4 \\
B \texttt{aegis2\_\allowbreak{}prompt} & accuracy & 72.1 & 70.4 & 70.2 & 65.2 & 66.0 & 73.4 & 68.8 \\
B \texttt{bipia\_\allowbreak{}injection} & accuracy & 79.5 & 84.1 & 72.7 & 95.5 & 50.0 & 36.4 & 93.2 \\
B \texttt{browsesafe} & accuracy & 60.6 & 61.0 & 56.6 & 60.2 & 59.4 & 55.4 & 54.2 \\
B \texttt{cosapien\_\allowbreak{}policy} & accuracy & 84.8 & 81.8 & 84.8 & 84.8 & 75.7 & 72.6 & 69.6 \\
B \texttt{jailbreak\_\allowbreak{}wild} & accuracy & 62.9 & 48.5 & 63.3 & 56.6 & 57.5 & 60.4 & 58.5 \\
B \texttt{jbb\_judge} & auroc & 95.9 & 94.8 & 95.8 & 96.2 & 93.6 & 94.8 & 93.3 \\
B \texttt{xstest} & auroc & 99.6 & 99.2 & 99.3 & 98.6 & 97.6 & 98.0 & 96.3 \\
C \texttt{contextual\_\allowbreak{}judge} & accuracy & 18.3 & 19.2 & 19.5 & 28.6 & 19.2 & 15.4 & 17.7 \\
C \texttt{faithbench} & accuracy & 27.6 & 11.2 & 19.7 & 25.0 & 18.4 & 11.8 & 7.2 \\
C \texttt{judgebench} & accuracy & 58.3 & 64.8 & 59.0 & 55.4 & 44.7 & 52.5 & 50.9 \\
C \texttt{llmbar} & accuracy & 64.4 & 76.4 & 58.9 & 64.9 & 69.4 & 67.9 & 46.4 \\
C \texttt{processbench} & accuracy & 72.0 & 71.2 & 67.3 & 67.1 & 64.7 & 61.3 & 60.2 \\
C \texttt{rewardbench} & accuracy & 91.2 & 89.9 & 91.0 & 92.8 & 87.5 & 87.3 & 87.7 \\
C \texttt{rewardbench2} & accuracy & 77.3 & 75.9 & 72.5 & 74.4 & 77.4 & 74.4 & 68.6 \\
C \texttt{squad2\_\allowbreak{}answerable} & accuracy & 57.2 & 83.7 & 52.5 & 67.8 & 75.4 & 50.6 & 64.4 \\
D \texttt{agentreward\_\allowbreak{}success} & accuracy & 53.6 & 56.2 & 52.2 & 38.8 & 55.1 & 56.5 & 46.0 \\
D \texttt{bfcl\_\allowbreak{}relevance} & accuracy & 80.7 & 77.3 & 77.3 & 83.0 & 75.0 & 70.5 & 73.9 \\
D \texttt{mind2web\_\allowbreak{}element} & accuracy & 90.5 & 88.5 & 89.6 & 78.5 & 79.2 & 83.2 & 74.8 \\
E \texttt{cuad\_clause} & accuracy & 72.5 & 65.6 & 76.2 & 63.7 & 63.7 & 63.7 & 63.7 \\
E \texttt{folio\_\allowbreak{}validation} & accuracy & 63.2 & 76.5 & 61.8 & 74.3 & 61.0 & 67.6 & 55.9 \\
E \texttt{legalbench\_\allowbreak{}mix} & accuracy & 61.0 & 62.3 & 63.8 & 64.2 & 61.6 & 63.3 & 58.8 \\
E \texttt{primevul\_\allowbreak{}pair} & pair accuracy & $-$25.1 & $-$24.5 & $-$25.1 & $-$27.5 & $-$23.2 & $-$29.3 & $-$26.7 \\
F \texttt{label\_\allowbreak{}errors} & accuracy & 26.7 & 21.9 & 29.3 & 21.3 & 23.1 & 24.9 & 26.7 \\
G \texttt{entity\_\allowbreak{}match\_\allowbreak{}abt\_\allowbreak{}buy} & auroc & 99.2 & 99.3 & 99.2 & 97.9 & 99.1 & 98.8 & 98.8 \\
G \texttt{entity\_\allowbreak{}match\_\allowbreak{}amazon\_\allowbreak{}google} & auroc & 93.0 & 94.1 & 92.8 & 92.2 & 92.8 & 92.6 & 91.5 \\
G \texttt{nevir} & pair accuracy & 60.8 & 73.6 & 57.1 & 57.1 & 61.3 & 65.1 & 64.0 \\
G \texttt{paws} & accuracy & 80.0 & 88.3 & 78.6 & 71.6 & 67.7 & 67.1 & 65.9 \\
G \texttt{rerank\_\allowbreak{}nfcorpus} & ndcg@10 & 34.2 & 35.0 & 33.5 & 33.2 & 30.2 & 33.1 & 33.1 \\
G \texttt{rerank\_\allowbreak{}scifact} & ndcg@10 & 80.3 & 79.6 & 80.7 & 80.7 & 77.9 & 81.2 & 78.7 \\
\end{longtable}
\endgroup

\begin{table}[!htbp]
\renewcommand{\thetable}{D4}
\centering
\caption{\textbf{What a thought fixes and breaks: it fixes 2,187 to 2,600 items at every size, and only at 27B does its gain grow from level 1 to level 3}, 7,800 items per checkpoint. Fixed: wrong in one pass and right after the thought, broken: the reverse. Net change in points with a paired 95\% interval, and at level 1 and level 3 of the 13 families. Thoughts ended: share that ended by themselves within the limit of 4,096 tokens. Last column: accuracy after the thought on the items whose thought was cut at the limit. Source: \texttt{v1\_\allowbreak{}1/\allowbreak{}analysis/\allowbreak{}out/\allowbreak{}t6\_\allowbreak{}thinking\_\allowbreak{}long.\allowbreak{}csv}.}\label{tab:D4}
{\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrrrrr}
\toprule
\textbf{system} & {\begin{tabular}[b]{@{}r@{}}\textbf{one}\\\textbf{pass}\end{tabular}} & \textbf{thought} & \textbf{fixed} & \textbf{broken} & \textbf{net change} & {\begin{tabular}[b]{@{}r@{}}\textbf{level}\\\textbf{1}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{level}\\\textbf{3}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{thoughts}\\\textbf{ended}\\\textbf{(\%)}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{accuracy if cut}\\\textbf{at the limit}\end{tabular}} \\
\midrule
ours 27B-R & 70.3 & 97.9 & 2,187 & 38 & +27.6 {[}+26.6, +28.6{]} & +14.0 & +39.2 & 97.8 & 89.5 (172 items) \\
ours 9B-R & 53.6 & 84.0 & 2,600 & 230 & +30.4 {[}+29.4, +31.4{]} & +33.0 & +24.7 & 62.2 & 71.8 (2,946 items) \\
ours 4B-R & 51.2 & 80.6 & 2,546 & 255 & +29.4 {[}+28.3, +30.4{]} & +30.6 & +24.7 & 64.9 & 68.9 (2,737 items) \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\clearpage
\begin{figure}[!htbp]
\renewcommand{\thefigure}{D1}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/figD1_pair_by_level.pdf}
\caption{Pair accuracy falls from level 1 to level 3 for every system. Pair accuracy by level, pooled over the 13 families, for the 27B systems and our released 4B, with 95\% intervals. Blue: our checkpoints, orange: other decision models. Data: \texttt{figures/\allowbreak{}figD1\_\allowbreak{}pair\_\allowbreak{}by\_\allowbreak{}level.\allowbreak{}csv}.}\label{fig:D1}
\end{figure}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{D2}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/figD2_tracks.pdf}
\caption{The tracks order the systems alike, but only the core track separates the three at the top. Core pair accuracy against the reference total for the 15 systems with runs on both tracks, with 95\% intervals. Our released 9B and 9B-D share a reference total of 53.1 and lie 3.0 points apart in pair accuracy, and our released 4B and 4B-D lie next to each other. Blue: our checkpoints, orange: other decision models. Data: \texttt{figures/\allowbreak{}figD2\_\allowbreak{}tracks.\allowbreak{}csv}, correlation: \texttt{v1\_\allowbreak{}1/\allowbreak{}derived/\allowbreak{}track\_\allowbreak{}correlation.\allowbreak{}md}.}\label{fig:D2}
\end{figure}

\section{Audit of the generators}\label{sec:E}

\begin{table}[!htbp]
\renewcommand{\thetable}{E1}
\centering
\caption{\textbf{Every core family of version 1.1 passes every audit check} (\texttt{gen\_\allowbreak{}v4/\allowbreak{}audit\_\allowbreak{}v3.\allowbreak{}py} and \texttt{gen\_\allowbreak{}v4/\allowbreak{}solve\_\allowbreak{}all.\allowbreak{}py}, run on the items of version 1.1, \texttt{gen\_\allowbreak{}v4/\allowbreak{}AUDIT.\allowbreak{}md}). Ref: the larger of the majority rate, the share of the most frequent gold position and chance. Options and question + options: cross-validated bag-of-words regressions that see only the options, or the question and the options, with the members of a group in one fold. Length and lines: best single threshold on the characters and on the lines of the state (yes/no families). State words: the same regression on the words of the state, for information. Domains: distinct domains (-- where the family records none). Solver: agreement of the independent solver with the keys of version 1.1, and for the three families whose items did not change also on a second set drawn with seed 1.}\label{tab:E1}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{family} & \textbf{ref} & \textbf{options} & {\begin{tabular}[b]{@{}r@{}}\textbf{question}\\\textbf{+}\\\textbf{options}\end{tabular}} & \textbf{length} & \textbf{lines} & {\begin{tabular}[b]{@{}r@{}}\textbf{state}\\\textbf{words}\end{tabular}} & \textbf{domains} & \textbf{solver} \\
\midrule
\texttt{perm\_\allowbreak{}inherit} & 0.500 & 0.472 & 0.472 & 0.503 & 0.500 & 0.500 & 5 & 600 / 600, 600 / 600 \\
\texttt{sched\_\allowbreak{}conflict} & 0.500 & 0.464 & 0.464 & 0.502 & 0.500 & 0.527 & 5 & 600 / 600 \\
\texttt{triage\_\allowbreak{}order} & 0.200 & 0.213 & 0.213 & -- & -- & 0.193 & 6 & 600 / 600 \\
\texttt{clause\_\allowbreak{}change} & 0.333 & 0.253 & 0.253 & -- & -- & 0.305 & 6 & 600 / 600, 600 / 600 \\
\texttt{dep\_resolve} & 0.500 & 0.469 & 0.469 & 0.503 & 0.500 & 0.500 & 5 & 600 / 600, 600 / 600 \\
\texttt{ledger\_\allowbreak{}reconcile} & 0.167 & 0.146 & 0.144 & -- & -- & 0.128 & 5 & 600 / 600 \\
\texttt{record\_rule} & 0.122 & 0.111 & 0.110 & -- & -- & 0.116 & 8 & 600 / 600 \\
\texttt{answerable\_\allowbreak{}facts} & 0.500 & 0.469 & 0.469 & 0.507 & 0.500 & 0.489 & -- & 600 / 600 \\
\texttt{policy\_case} & 0.333 & 0.260 & 0.260 & -- & -- & 0.238 & 4 & 600 / 600 \\
\texttt{log\_\allowbreak{}count\_\allowbreak{}check} & 0.500 & 0.460 & 0.460 & 0.503 & 0.500 & 0.457 & -- & 600 / 600 \\
\texttt{state\_goal} & 0.500 & 0.500 & 0.500 & 0.505 & 0.500 & 0.500 & 5 & 600 / 600 \\
\texttt{toolcall\_\allowbreak{}valid} & 0.500 & 0.500 & 0.500 & 0.507 & 0.508 & 0.527 & -- & 600 / 600 \\
\texttt{filter\_\allowbreak{}match} & 0.500 & 0.473 & 0.473 & 0.503 & 0.500 & 0.511 & 4 & 600 / 600 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

Every family passes every required check: the regressions on the options and on the question with
the options do not beat the reference by more than 3 points, no length or line threshold leaves 0.50
$\pm$ 0.02, the gold positions are balanced, and no state is repeated. No word of frequency 20 or
more is more than twice as frequent in one class as in the other in any yes/no or three-way family,
and no row of our 135,006 procedural training rows shares two 13-word sequences with a core item.

\textbf{What version 1.1 changed.} The two AI reviewers answered 65 items of version 1.0 and agreed
with every key, but they listed defects that change no key and yet give a model a cue or make an
item read as made up. Version 1.1 rebuilt ten families with corrected generators, which remove these
defects and a few that the new independent solvers found, and measured each defect on both versions
with the same script (Table~\ref{tab:E2}). Some properties stay as they are. Coherent policies leave
a mild prior in \texttt{policy\_case}, where calling the least risky-looking case of a policy
approve is right in 44\% of the triples against a chance of 33\%. In
\texttt{sched\_\allowbreak{}conflict} each positive still sits on the limit its negative crosses,
and in \texttt{toolcall\_\allowbreak{}valid} a reader who checks only the schema and the rules of
the tool reaches 0.917, since only the near misses of a requested value need the request.

\begin{table}[!htbp]
\renewcommand{\thetable}{E2}
\centering
\caption{\textbf{Version 1.1 removes the defects found in version 1.0 by the two AI reviewers and by the independent solvers.} Measured with the same script on both versions (\texttt{gen\_\allowbreak{}v4/\allowbreak{}AUDIT.\allowbreak{}md}).}\label{tab:E2}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1385}}>{\raggedright\arraybackslash}p{\mdw{0.4531}}>{\raggedright\arraybackslash}p{\mdw{0.3943}}}
\toprule
\textbf{family} & \textbf{defect in version 1.0} & \textbf{change in version 1.1} \\
\midrule
\texttt{filter\_\allowbreak{}match} & requests that count days did not say how, a constraint worded so that it could name another field, implausible records such as a list price below the price & the day-count rule stated in every such request, unambiguous field wordings, prices and specs inside the range of their category \\
\texttt{state\_goal} & a description of the steps that was false for some step in most items, pseudo-word names, and a cue in 66 negatives whose failing condition no step touched & a true description, ordinary names in five domains, goal-directed traces, the cue removed, the pairs marked as groups \\
\texttt{policy\_case} & rules against the direction of risk (approve because consent is missing), dead and near-duplicate rules, inconsistent case records & every rule reads its condition in the direction of its outcome, no dead or duplicate rule, consistent records \\
\texttt{record\_rule} & derived fields that disagree outside the planted violation, the status convention of reference lists left implicit & consistent background records, the status convention written in every state that needs it \\
\texttt{triage\_\allowbreak{}order} & time columns that contradict each other, a class-first reading that gave the key in 37\% of the level-1 items & consistent times, the class as the first written rule at level 1, the shortcut capped at levels 2 and 3 \\
\texttt{log\_\allowbreak{}count\_\allowbreak{}check} & claims such as ``exactly 1 ERROR entries'' and claims open to an at-least reading & every claim says exactly, with the right noun, and stated counts balanced within each level \\
\texttt{sched\_\allowbreak{}conflict} & 60\% of the negatives at levels 2 and 3 decided by a cheap check of hours, seats or equipment & 30\% at level 2 and 15\% at level 3, the rest planted in the booking list \\
\texttt{answerable\_\allowbreak{}facts} & a quarter of the founding years at one clamped value, two crossed dials instead of a level ladder & founding years spread over a wide range, a level ladder \\
\texttt{ledger\_\allowbreak{}reconcile} & a ledger named in two ways within one item, no rule for negative amounts & one name per ledger, the deduction rule stated for both signs \\
\texttt{toolcall\_\allowbreak{}valid} & request words equal to a parameter name without referring to it, a few filler sentences repeated across many items & no such words, many more neutral filler sentences, the pairs marked as groups \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

